Think Right, Not More: Test-Time Scaling for Numerical Claim Verification

Fact-checking real-world claims, particularly numerical claims, is inherently complex that require multistep reasoning and numerical reasoning for verifying diverse aspects of the claim. Although large language models (LLMs) including reasoning models have made tremendous advances, they still fall short on fact-checking real-world claims that require a combination of compositional and numerical reasoning. They are unable to understand nuance of numerical aspects, and are also susceptible to the reasoning drift issue, where the model is unable to contextualize diverse information resulting in misinterpretation and backtracking of reasoning process. In this work, we systematically explore scaling test-time compute (TTS) for LLMs on the task of fact-checking complex numerical claims, which entails eliciting multiple reasoning paths from an LLM. We train a verifier model (VERIFIERFC) to navigate this space of possible reasoning paths and select one that could lead to the correct verdict. We observe that TTS helps mitigate the reasoning drift issue, leading to significant performance gains for fact-checking numerical claims. To improve compute efficiency in TTS, we introduce an adaptive mechanism that performs TTS selectively based on the perceived complexity of the claim. This approach achieves 1.8x higher efficiency than standard TTS, while delivering a notable 18.8% performance improvement over single-shot claim verification methods. Our code and data can be found at https://github.com/VenkteshV/VerifierFC

==> 03-framework.tex <==
\section{Methodology}
\label{sec:methods}

==> algo-SUNAR.tex <==
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\begin{figure}[t]\vspace{-1em}
% \small
\begin{algorithm}[H]
  \SetAlgoLined
\caption{The \name{} Algorithm} 
\label{alg: main}
% \small
\begin{algorithmic}[1]
\small
\Require Initial retrieved list $R$, batch size $b$, re-ranking budget $c$, document graph $G$
\Ensure Re-Ranked pool $R^+$
\State $R^+ \gets \emptyset$ \Comment{Re-Ranking results}
\State $C \gets R$ \Comment{Candidate pool}
\State $N \gets \emptyset$ \Comment{Neighbor pool}
% \State\HiLi $\Call{SetAff}{.} \gets 0$ \Comment{Initialize expected affinity scores}
\Do
  \State $B \gets$ \Call{Score}{top $b$ from $C$, subject to $c$} 
  
  % \Comment{Ranker}
    \State  $\{sa_1...sa_m\} \gets \phi(\bP_{LLM}(sq_1,B))$   
    % \Comment{multiple responses (Eq 2)}

    \State  $\{ac_1..ac_s\} \gets \sigma(sa_1..sa_m)$ 
    % \Comment{semantic clustering}
    \Comment{Clustering}

    \State
 \State $B \gets$ \Call{rescore}{$B$,$1/s$} \Comment{Rescore batch}
 % using number of semantic sets }
  \State $R^+ \gets R^+ \cup B$ \Comment{Add batch to results}

\State
  \State 
  // Discard Batches
  \State $R \gets R \setminus B$ 
  % \Comment{Discard batch from ranking}
  \State $N \gets N \setminus B$ 
  % \Comment{Discard batch from nbr.}
  % \State $S \gets$ \Call{Select}{top $s$ from $R_1$} \Comment{Select top $s$ ranked docs}
  \State $N \gets N \cup (\Call{Neighbours}{B, G} \setminus R^+$) 
  % \hspace{-0.5em}\Comment{Update frontier}
% \State\HiLii $\Call{SetAff}{d} \gets \Call{SetAff}{d} + \Call{SetAff}{d,R_1}, \quad \forall d \in F$ \Comment{\small{Update Exp. Aff. Scores using (\ref{eq:eaffm})}}
% \normalsize

\State
\State //Alternate $R$ and $N$
  \State $C \gets \begin{cases} 
      R & \text{if}\; C = F   \\
      N  & \text{if}\; C = N \\
   \end{cases}$ 
   % \hspace{-2em}\Comment{Alternate $R_0$ and $N$}
\doWhile{$|R^+| < c$}
%\State $R_1 \gets R_1 \cup \Call{Backfill}{R_0, R_1}$ \Comment{Backfill remaining items}
\end{algorithmic}
\end{algorithm}
\end{figure}


==> algo-sunar-v2.tex <==
\begin{algorithm}[H]
  \SetAlgoLined
\caption{The \name{} Algorithm} 
\label{alg: main}
\begin{algorithmic}[1]
\Require Initial retrieved list $R$, batch size $b$, re-ranking budget $c$, document graph $G$
\Ensure Re-Ranked pool $R^+$

  // Initialize re-ranking results
  \State $R^+ \gets \emptyset$

  // Initialize re-ranking pool
  \State $C \gets R$

  // Initialize neighbor pool
  \State $N \gets \emptyset$

\doWhile{$|R^+| < c$}

    // Ranker: Select top $b$ documents, subject to budget $c$
    \State $B \gets$ \Call{Score}{top $b$ from $P$, subject to $c$}

    // Generate multiple responses using language model
    \State $\{sa_1...sa_m\} \gets \phi(\bP_{LLM}(sq_1,B))$

    // Apply semantic clustering on the responses
    \State $\{ac_1..ac_s\} \gets \sigma(sa_1..sa_m)$

    // Rescore batch using number of semantic sets
    \State $B \gets$ \Call{rescore}{$B$, $1/s$}

    // Add batch to re-ranked results
    \State $R^+ \gets R^+ \cup B$

    // Remove batch from initial ranking
    \State $R \gets R \setminus B$

    // Remove batch from neighbor pool
    \State $N \gets N \setminus B$

    // Update frontier by adding neighbors of batch, excluding already re-ranked
    \State $N \gets N \cup (\Call{Neighbours}{B, G} \setminus R^+)$

    // Alternate between re-ranking pool and neighbor pool
    \State $C \gets \begin{cases} 
        R & \text{if}\; C = F \\
        N & \text{if}\; C = N \\
    \end{cases}$

\endDoWhile

\end{algorithmic}
\end{algorithm}

==> auto-cot-prompt.tex <==
\begin{table}[htb!!]
\begin{tcolorbox}[title=Prompt: Auto Chain of Thought]
\small
\textbf{\ding{228} \textsc{System Message}}: You are tasked with providing rationale and answers to timeline-based queries about various subjects. \newline
Your reply should try to be as complete as possible. Think of the subject's past and contributions. Try to think step by step. Write down your thinking process. \newline
After you provide an answer, you will next be tasked to extract the timelines from there, which should answer the first question best. 

The timeline should be structured like this: \vspace{0.2cm}

Each answer should be structured as a list, with different entries for each subject or title. Each entry must include the years corresponding to the following the title or subject. \vspace{0.2cm}

Please adhere to the following structure in your responses: \\
- Write the title or name first, exactly as it would appear in a formal context such as Wikipedia. \\
- Follow the title or name with a colon and then the years. \\
- Represent a range of years by using a short dash. \\
- Separate multiple years or ranges with a comma and a space. \\
- End each entry with a comma, except for the last entry. \\
- If the current year is relevant to the query, use "2024" instead of "present". \\
- Each answer should be on a new line, with no additional characters or explanations. \\
- Ensure the completeness and correctness of your answers. Try to be as complete as possible. \\
- If provided examples, follow the examples structure and reasoning style. \vspace{0.2cm}

\textbf{Example response format:} \\
\texttt{Title or Name: year1-year2, year3} \\
\texttt{Title or Name: Years}, \vspace{0.2cm}

\textbf{\ding{228} \textsc{User Message (Example)}}: \textit{List all political positions Greg Abbott held to this day.} \\

% Indicate automatic rationale generation below
\textbf{\ding{228} \textsc{Assistant Message (Auto-Generated Rationale)}}: 
 \textit{Greg Abbott is a prominent American politician and officeholder. He first served as Justice of the Supreme Court in Texas from 1996 to 2001. In 2002, Abbott was elected as the 50th Attorney General of Texas. In 2014, he announced his candidacy for Governor of Texas, winning the election and taking office in 2015. Abbott has continued to serve as Governor to this day. Additionally, between 2019 and 2020, Abbott was the Chair of the Republican Governors Association.} \newline  

\textbf{\ding{228} \textsc{User Message}}: \textit{Extract the timeline, including both years and answers from your previous answer now. }\\ \\ 
\textbf{\ding{228} \textsc{Assistant Message (Example)}}:
\textit{"Governor of Texas": 2015-2024,} \newline
\textit{"Chair of the Republican Governors Association": 2019-2020,} \newline
\textit{"50th Attorney General of Texas": 2002-2015,} \newline
\textit{"Justice of the Supreme Court of Texas": 1996-2001} \\ 

\textbf{\ding{228} \textsc{User Message}}: \textit{List all political positions Brian Pallister held to this day.} 
\end{tcolorbox}
\captionof{figure}{Auto COT prompt setup (closed book setting)}
\label{fig:timeline_rationale_prompt}
\end{table}


==> error_analysis.tex <==

\begin{table*}[h!]
    \centering
    \begin{tabular}{p{7.4cm} p{7.4cm}}
    \toprule
        %     \multicolumn{2}{l}{ {\color{olive}\textit{CONTENT WARNING: potentially objectionable content}} } \\
        % \midrule
    \multicolumn{2}{l}{\ding{228} \textbf{Query}: \texttt{List all teams  Alan Kirby played to this day.}} \\
    \midrule
    \textbf{Expected Answer} & \textbf{\textbf{Generated Answer} } \\
    \midrule

    \vspace{-10pt} % Manually adjust vertical space
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
        \item Aston Villa F.C.: 1996-1998, 1994-1996
        \item Johnville F.C. (Waterford): 1994
        \item Republic of Ireland under-21 national football team: 1998
        \item Waterford United F.C.: 1999-2001
        \item League of Ireland XI: 2010
        \item Longford Town F.C.: 2001-2006, 2012
        \item St Patrick's Athletic F.C.: 2007-2008
        \item Sporting Fingal F.C.: 2009-2010
        \item Sligo Rovers F.C.: 2011
    \end{itemize}
    
    
    
            & I apologize, but I couldn't find any information on a person named Alan Kirby playing for any football teams. If you meant someone else or provided incorrect information, please let me know and I'll be happy to help.  \\
    
    \bottomrule
    \end{tabular}
    \caption{Example of query that the model is not able to answer. Generated with Meta Llama 3 with manual 3-shot prompting. }
    \label{tab:refusal_example}
    
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{p{7.4cm} p{7.4cm}}
    \toprule
    \multicolumn{2}{l}{\ding{228} \textbf{Query}: \texttt{List all teams Alan Kirby played to this day.}} \\
    \midrule
    \textbf{Expected Answer} & \textbf{Generated Answer} \\
    \midrule
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
        \item Aston Villa F.C.: 1996-1998, 1994-1996
        \item Johnville F.C. (Waterford): 1994
        \item Republic of Ireland under-21 national football team: 1998
        \item Waterford United F.C.: 1999-2001
        \item League of Ireland XI: 2010
        \item Longford Town F.C.: 2001-2006, 2012
        \item St Patrick's Athletic F.C.: 2007-2008
        \item Sporting Fingal F.C.: 2009-2010
        \item Sligo Rovers F.C.: 2011
    \end{itemize}
    
    &
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
    \item Leeds United F.C.: 1995-2001, 2000 
    \item England national under-21 football team: 1999 
    \item Huddersfield Town A.F.C.: 2001-2004
    \item Rotherham United F.C.: 2004-2006 
    \item Doncaster Rovers F.C.: 2006-2008 
    \item Grimsby Town F.C.: 2008-2010 
    \item Bradford City A.F.C.: 2010-2011 
    \item Gainsborough Trinity F.C.: 2011-2012 
    \item Harrogate Railway Athletic F.C.: 2012-2013 
    \item Farsley Celtic F.C.: 2013-2014 
    \item York City F.C.: 2014-2015
    \item Brighouse Town A.F.C.: 2015-2016 
    \item AFC Emley F.C.: 2016-2017
    \item Garforth Town A.F.C.: 2017-2018 
    \item Liversedge F.C.: 2018
    \end{itemize}
    
    \\
    \bottomrule
    \end{tabular}
    \caption{Example of model answer with incorrect details. }
    \label{tab:hallucination_model_answer}
\end{table*}
\begin{table*}[h!]
    \centering
    \begin{tabular}{p{7.4cm} p{7.4cm}}
    \toprule
    \multicolumn{2}{l}{\ding{228} \textbf{Query}: \texttt{List all political positions Ulf Kristersson held to this day.}} \\
    \midrule
    \textbf{Expected Answer} & \textbf{Generated Answer} \\
    \midrule
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
        \item Prime Minister of Sweden: 2022-2024
        \item \textcolor{red}{Leader of the Moderate Party: 2017-2024}
        \item Leader of the Opposition: 2017-2022
        \item Minister for Social Security: 2010-2014
        \item Chairman of the Moderate Youth League: 1988-1992
        \item \textcolor{red}{Member of the Riksdag: 2014-2024, 1991-2000}
    \end{itemize}
    
    &
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
    \item \textcolor{red}{Leader of the Moderate Party: 2017-2024}
    \item \textcolor{red}{Member of the Riksdag: 2006-2021, 2022-2024}
    \end{itemize}
    
    \\
    \bottomrule
    \end{tabular}
    \caption{Example of incomplete answer}
    \label{tab:incomplete_answer}
\end{table*}


==> exemplars-qualitative.tex <==



\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Question}: A cat chases a rat 6 hours after the rat runs. cat takes 4 hours to reach the rat. If the average speed of the cat is 90 kmph, what s the average speed of the rat?
\\ & \textbf{Options}: ['A)32kmph', 'B)26kmph', 'C)35kmph', 'D)36kmph', 'E)32kmph']
\\ & \textbf{Rationale:} Cat take 10 hours and rat take 4 hours...then Distance is 90*4.so speed of rat is (90*4)/10 = 36kmph 
\textbf{Answer: D}
 \\\cline{2-2}
 & \textbf{Question:}  A business executive and his client are charging their dinner tab on the executive's expense account.The \dots?
 \\ & \textbf{Options}: ['A)69.55\$', 'B)50.63\$', 'C)60.95\$', 'D)52.15\$', 'E)53.15'] \\
 & \textbf{Rationale}:  let x is the cost of the food
1.07x is the gross bill after including sales tax
1.15* 1.07x=75 \textbf{Answer}: C \\\cline{2-2}
 & \textbf{Question:}John and David were each given X dollars in advance for each day they were expected to perform at a community festival. John eventually,\dots? 
 \\ &\textbf{Options}: 'A)11Y', 'B)15Y', 'C)13Y', 'D)10Y', 'E)5Y' \textbf{Rationale:} \dots  \textbf{Answer:} A\\\cline{2-2}
  & \textbf{Question:}A contractor undertakes to do a piece of work in 40 days. He engages 100 men at the beginning and 100 more after 35 days and completes the work in stipulated time. If he had not engaged the additional men, how many days behind schedule would it be finished?? \\
 & \textbf{Options}: 'A)2', 'B)5', 'C)6', 'D)8', 'E)9'
  \textbf{Rationale:}  [(100$\times$ 35)+(200$\times$ 5)] men can finish the work in 1 day
therefore 4500 men can finish the work in 1 day. 100 men can finish it in  $\frac{4500}{100}$ = 45 days.
This is 5 days behind Schedule 
  \textbf{Answer:} A\\\cline{2-2}
    & \textbf{Question:} A can do a job in 9 days and B can do it in 27 days. A and B working together will finish twice the amount of work in ------- days? \\
 & \textbf{Options}: 'A)22 days', 'B)18 days', 'C)22 6/2 days', 'D)27 days', 'E)9 days'
  \textbf{Rationale:} 1/9 + 1/27= 3/27 = 1/9
9/1 = 9*2 =18 day
  \textbf{Answer:} B\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Question}: The average age of three boys is 15 years and their ages are in proportion 3:5:7. What is the age in years of the youngest boy?
\\ \colorg & \colorg \textbf{Options}: ['A)9', 'B)10', 'C)11', 'D)12', 'E)13']
\\\colorg & \colorg\textbf{Rationale:}3x + 5x + 7x = 45,
x =3,
3x = 9
\textbf{Answer: A}
 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}  Can you deduce the pattern and find the next number in the series? $6, 14, 26, 98$?

  \textbf{Options}: [''A)276', 'B)277', 'C)278', 'D)279', 'E)None of these']] \\\colorg
 & \colorg\textbf{Rationale}:  $6 = 1^1 + 2^1 + 3^1, 
14 = 1^2 + 2^2 + 3^2,
36 = 1^3 + 2^3 + 3^3,
98 = 1^4 + 2^4 + 3^4$
Thus the next number 
 \textbf{Answer}: A \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}In covering a distance of 42 km, A takes 2 hours more than B. If A doubles his speed, then he would take 1 hour less than B. A's speed is:? 
\\ \colorg & \colorg \textbf{Options}: 'A)5 km/h', 'B)7 km/h', 'C)10 km/h', 'D)15 km/h', 'E)25 km/h' \textbf{Rationale:} Let A's speed be X km/hr.
Then, 42/x - 42/2x = 3
6x = 42
x = 7 km/hr \textbf{Answer:} B\\\cline{2-2}\colorg
  &\colorg \textbf{Question:}Find  the number which when multiplied by 15 is increased by 196. \\\colorg
 &\colorg \textbf{Options}: 'A)14', 'B)20', 'C)26', 'D)28', 'E)30'
  \textbf{Rationale:}  Solution
Let the number be x .
Then, 15x - x = 196
‹=›14x = 196
x ‹=› 14 
  \textbf{Answer:} A\\\cline{2-2}\colorg
    & \colorg\textbf{Question:} A certain sum of money at simple interest amounted Rs.980 in 3 years at 5\% per annum, find the sum? \\\colorg
 & \colorg\textbf{Options}: 'A)867', 'B)855', 'C)299', 'D)852', 'E)903'
  \textbf{Rationale:} 980 = P [1 + (3*5)/100]
P = 852 
  \textbf{Answer:} D\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\aqua{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_aquarat}
%\vspace{-0.25cm}
\end{table*}





















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Table}: | increase ( decrease ) |
average yield | 2.75\% ( 2.75 \% ) |
volume | 0.0 to 0.25 |
energy services | 2013 |
fuel recovery fees | 0.25 |
recycling processing and commodity sales | 0.25 to 0.5 |
acquisitions / divestitures net | 1.0 |
total change | 4.25 to 4.75\% ( 4.75 \% ) |
\\ & \textbf{Question}: what is the ratio of the acquisitions / divestitures net to the fuel recovery fees as part of the expected 2019 revenue to increase
\\ & \textbf{Rationale:} ans=( 1.0 / 0.25 )
\textbf{Answer: }  The answer is 4
 \\\cline{2-2}
 & \textbf{Table:}  ( in millions ) | 2009 | 2008 | 2007 |
sales and transfers of oil and gas produced net of production andadministrative costs |  -4876 ( 4876 ) |  -6863 ( 6863 ) |  -4613 ( 4613 ) |
\dots
 \\ & \textbf{Question}: were total revisions of estimates greater than accretion of discounts?
\\
 & \textbf{Rationale}: \dots   \textbf{Answer}: The answer is yes  \\\cline{2-2}
 & \textbf{Table:} | 2007 | 2008 | change |
capital gain distributions received | 22.1 |  5.6 | -16.5 ( 16.5 ) |
other than temporary impairments recognized | -.3 ( .3 ) | -91.3 ( 91.3 ) | -91.0 ( 91.0 ) |
net gains ( losses ) realized onfund dispositions | 5.5 | -4.5 ( 4.5 ) | -10.0 ( 10.0 ) |
net gain ( loss ) \dots
 \\ &\textbf{Question}: what percentage of tangible book value is made up of cash and cash equivalents and mutual fund investment holdings at december 31 , 2009?
\textbf{Rationale:} ( 1.4 / 2.2 )  \textbf{Answer:}  The answer is 64\%\\\cline{2-2}
  & \textbf{Table:} in millions | 2009 | 2008 | 2007 |
sales | 5680 | 6810 | 6530 |
operating profit | 1091 | 474 | 839 |
\\
 & \textbf{Question}: north american printing papers net sales where what percent of total printing paper sales in 2009?
   \textbf{Rationale:} x0=( 2.8 * 1000 ), ans=( x0 * 5680 )
  \textbf{Answer:} The answer is 49\%\\\cline{2-2}
    & \textbf{Table:}  in millions | december 312015 | december 312014 |
total consumer lending | 1917 | 2041 |
total commercial lending | 434 | 542 |
total tdrs | 2351 | 2583 |
nonperforming | 1119 | 1370 |
\dots
 \\
 & \textbf{Question}: what was the change in specific reserves in alll between december 31 , 2015 and december 31 , 2014 in billions?
  \textbf{Rationale:} ( .3 - .4 )
  \textbf{Answer:}  The answer is -0.1\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Table}: | 2008 | 2007 |
balance at beginning of year | 23.2 | 56.4 |
additions due to acquisition of allied | 582.9 | 2014 |
additions based on tax positions related to current year | 10.6 | 16.3 |
reductions for tax positions related to the current year | -5.1 ( 5.1 ) | -17.2 ( 17.2 ) |
\dots
\\ \colorg & \colorg \textbf{Question}: in 2008 what was the change in the gross unrecognized tax benefits in millions
\\\colorg & \colorg\textbf{Rationale:}  (611.9 - 23.2 )
\textbf{Answer: } The answer is 588.7
 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} december 31 2004 | 1054 |
december 31 2005 | 1216 |
december 31 2006 | 1219 |
december 31 2007 | 2566 |
  \textbf{Question}: what was devon's average translation adjustments included in accumulated other comprehensive income ( in millions ) from 2004 through 2007?
\textbf{Rationale}: x0=( 1054 + 1216 ), x1=( x0 + 1219 ), x2=( x1 + 2566 ), ans=( x2 + 4 )
 \textbf{Answer}: The answer is 1513.75 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | 2016 | 2015 ( in thousands ) | 2014 |
share-based compensation expense | 30809 | 21056 | 29793 |
income tax benefit | 9879 | 6907 | 7126 |
\\ \colorg & \colorg \textbf{Question}:  how much percent did the income tax benefit increase from 2014 to 2016?
  \\\colorg  & \colorg  \textbf{Rationale:}  x0=( 9879 - 7126 ), ans=( x0 - 7126 )
 \textbf{Answer:} The answer is increased 38.6\%\\\cline{2-2}\colorg
  &\colorg \textbf{Table:}  in billions | 2018 |
january 1 |  33.3 |
issuances | 4.5 |
calls and maturities | -6.8 ( 6.8 ) |
other | -.1 ( .1 ) |
december 31 | 30.9 |
\\\colorg
 &\colorg \textbf{Question}: assuming all matured securities were pledged as collateral , how much should we assume came from the calls?
  \textbf{Rationale:}  ans=( 6.8 - 4.9 ) 
  \textbf{Answer:} The answer is 1.9 \\\cline{2-2}\colorg
    & \colorg\textbf{Table:}  in millions of dollars | u.s . | outside u.s . | december 31 2008 | december 31 2007 |
commercial and similar letters of credit | 2187 | 6028 | 8215 | 9175 |
 \dots\\\colorg
 & \colorg\textbf{Question}: what percentage of citigroup 2019s total other commitments as of december 31 , 2008 are outside the u.s.?
  \textbf{Rationale:}  ans=( 236931 / 1349500 )
  \textbf{Answer:} The answer is 18\%\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\fin{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_fin}
%\vspace{-0.25cm}
\end{table*}
















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Question}: Michael wants to dig a hole 400 feet less deep than twice the depth of the hole that his father dug. The father dug a hole at a rate of 4 feet per hour. If the father took 400 hours to dig his hole \dots ?
\\ & \textbf{Rationale:} Since the father dug a hole with a rate of 4 feet per hour, if the father took 400 hours digging the hole, he dug a hole 4*400 = 1600 feet deep. \dots Michael will have to work for 2800/4 = 700 hours.
\textbf{Answer:} 700
 \\\cline{2-2}
 & \textbf{Question:} When Erick went to the market to sell his fruits, he realized that the price of lemons had risen by $4$ for each lemon. The price of grapes had also increased by half the price that \dots?
 \\ & \textbf{Rationale}:  The new price for each lemon after increasing by $4$ is $8+4 =12$ For the 80 lemons, \dots Erick collected $140*9=1260$ From the sale of all of his fruits, Erick received $1260+960 =2220$.
 \\ & \textbf{Answer}: 2220 \\\cline{2-2}
 & \textbf{Question:}James decides to build a tin house by collecting 500 tins in a week. On the first day, he collects 50 tins. On the second day, he manages to collect 3 times that number. \dots? 
 \\ &\textbf{Rationale:} On the second day, he collected 3 times the number of tins he collected on the first day, which is $3*50 =150$ tins. \dots he'll need to collect $200/4=50$ tins per day to reach his goal. \\&\textbf{Answer:} 50\\\cline{2-2}
  & \textbf{Question:} Darrel is an experienced tracker. He can tell a lot about an animal by the footprints it leaves behind. Based on the impressions, he could tell the animal was traveling east at 15 miles per hour \dots ? \\
 & \textbf{Rationale:} If we let x be the amount of time, in hours, it will take for Darrel to catch up to the coyote, \dots If we subtract 1 x from each side, we get x=1, the amount of time in hours.
 \textbf{Answer:} 1\\\cline{2-2}
    & \textbf{Question:} Martha needs to paint all four walls in her 12 foot by 16 foot kitchen, which has 10 foot high ceilings \dots If Martha can paint 40 square feet per hour, how many hours will it take her to paint kitchen? 
  \\&\textbf{Rationale:} There are two walls that are 12' by 10' and two walls that are 16' by 10' \dots how many hours she needs to finish: 1680 sq ft / 40 sq ft/hour = 42 hours 
  \textbf{Answer:} 42\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Question}: The difference between the number of boys and girls in a tree planting event is 400. If there are 600 boys at the event, and the number of girls is more than the number of boys \dots ?
\\ \colorg & \colorg \textbf{Rationale:}  If there are 600 boys at the event, and the difference between boys and girls is 400, there are 600+400=1000 girls.
\dots 60\% of the total number of boys and girls at the event is 60/100*1600=960
\textbf{Answer:} 960
 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}  Casey is trying to decide which employee she wants to hire. One employee works for $\$20$ an hour. The other employee works for $\$22$ an hour, but Casey would also get a $\$6$/hour subsidy \dots ?
\\\colorg  & \colorg\textbf{Rationale}:  First find the weekly cost of the first employee: \$20/hour * 40 hours/week = 800/week \dots subtract the smaller weekly cost from the bigger weekly cost: \$800/week - \$640/week = 160/week.
 \textbf{Answer}: 160 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}Cara has 60 marbles in a bag. 20 of them are yellow, half as many are green, \dots If Cara picks a marble at random, what are the odds it's blue (expressed as a percentage)?
\\ \colorg & \colorg \textbf{Rationale:} First find the number of green marbles: 20 yellow marbles/2=10 green marbles. \dots find the percentage chance of getting a blue marble: 15 marbles/60 marbles*100=25\%.
\textbf{Answer:} 25\\\cline{2-2}\colorg
&\colorg \textbf{Question:} Samir just turned half the age Hania was 10 years ago. If in five years Hania will be 45 years old, what will Samir's age be five years from now?
 \\\colorg  &\colorg 
\textbf{Rationale:} If in five years, Hania will be 45 years old, currently she is 45-5=40 years old. Ten years ago, Hania was 40-10=30 years old. \dots In five years, Samir will be 15+5=20 years old. 
\textbf{Answer:} 20\\\cline{2-2}\colorg
& \colorg\textbf{Question:} If the normal hours of operation of Jean's business are 4 pm to 10p every day Monday through Friday, and from 6 pm to 10 pm on weekends, how many hours is the business open in a week?
\\\colorg
& \colorg \textbf{Rationale:} First, we find the number of hours per weekday by subtracting the smaller number from the larger one \dots We add these two totals together to find that 30+8=38 hours per week.
\textbf{Answer:} 38\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\gsm{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_gsm8k}
%\vspace{-0.25cm}
\end{table*}











\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Table}: | Name | Age (years)
| Jessica | 2
| Dalton | 7
| Kelsey | 5
| Lamar | 8
| Alexis | 2
 \textbf{Question}: A girl compared the ages of her cousins. What is the median of the numbers?
\textbf{Rationale:} Read the numbers from the table: 2, 7, 5, 8, 2.
First, arrange the numbers from least to greatest: 2, 2, 5, 7, 8.
Now find the number in the middle. The number in the middle is 5.
The median is 5.
\textbf{Answer: } 5
 \\\cline{2-2}
 & \textbf{Table:} | City | Number of houses sold 
| Melville | 878
| New Hamburg | 871
| Charles Falls | 881
| Pennytown | 817
\textbf{Question}: A real estate agent looked into how many houses were sold in different cities. Where were the fewest houses sold? \textbf{Rationale}: Find the least number in the table. \dots The least number is 817.
Now find the corresponding city. Pennytown corresponds to 817.
   \textbf{Answer}: 817  \\\cline{2-2}
 & \textbf{Table:} | Day | Number of new customers
| Saturday | 2
| Sunday | 2
| Monday | 9
| Tuesday | 4
| Wednesday | 10
| Thursday | 3
| Friday | 6
\textbf{Question}: A cable company analyst paid attention to how many new customers it had each day. What is the median of the numbers?
\textbf{Rationale:} Read the numbers \dots Now find the number in the middle. The number in the middle is 4.
The median is 4.
  \textbf{Answer:} 4 \\\cline{2-2}
  & \textbf{Table:} | Day | Number of cups
| Friday | 8
| Saturday | 4
| Sunday | 10
| Monday | 6
| Tuesday | 6
| Wednesday | 1
| Thursday | 0
 \textbf{Question}: Nancy wrote down how many cups of lemonade she sold in the past 7 days. What is the range of the numbers?
\textbf{Rationale:} Read the numbers from the table: 8, 4, 10, 6, 6, 1, 0. \dots Subtract the least number from the greatest number: 10-0=10. The range is 10.
\textbf{Answer:} 10\\\cline{2-2}
    & \textbf{Table:}  | Price | Quantity demanded | Quantity supplied
|\$700 | 9,800 | 22,600
|\$740 | 8,000 | 22,800
|\$780 | 6,200 | 23,000
|\$820 | 4,400 | 23,200
|\$860 | 2,600 | 23,400
\textbf{Question}: At a price of \$860, is there a shortage or a surplus?
 \textbf{Rationale:} At price of \$860, quantity demanded is less than quantity supplied. There is too much of the good or service for sale at that price. So, there is a surplus.
 \textbf{Answer:}  surplus\\
 \midrule

  
\colorg \static{} & \colorg \textbf{Table}: | Day | Number of tickets
| Monday | 36
| Tuesday | 43
| Wednesday | 46
| Thursday | 59
| Friday | 37
| Saturday | 46
| Sunday | 51
\textbf{Question}: The transportation company tracked the number of tickets sold in the past 7 days. What is the range of the numbers?
\textbf{Rationale:} Read the numbers from the table: 36, 43, 46, 59, 37, 46, 51. Find greatest number. The greatest number is 59. Find least
number. The least number is 36. Subtract least from the greatest number: 59 - 36 = 23.
The range is 23.
\textbf{Answer: } 23
 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | Stem | Leaf 
| 4 | 2, 7, 9, 9, 9
| 5 | 1
| 6 | 9
| 7 | 2, 2, 3, 3, 5
| 8 | 
| 9 | 0
\textbf{Question}:  A pottery factory kept track of the number of broken plates per shipment last week. How many shipments had exactly 73 broken plates?
\textbf{Rationale}:  For the number 73, the stem is 7, and the leaf is 3. Find the row where the stem is 7. In that row, count all the leaves equal to 3.
You counted 2 leaves, which are blue in the stem-and-leaf plot above. 2 shipments had exactly 73 broken plates.
\textbf{Answer}: 2 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | purple and red clay bead | \$0.02
| small pink bead | \$0.04
| pearl bead | \$0.07
| round silver bead | \$0.01
| brown cat's eye bead | \$0.08
| orange glass bead | \$0.07
\textbf{Question}:  Kylie has \$0.05. Does she have enough to buy a small pink bead and a purple and red clay bead?
\textbf{Rationale:}  Add the price of a small pink bead and the price of a purple and red clay bead: \$0.04 + \$0.02 = \$0.06
\$0.06 is more than \$0.05. Kylie does not have enough money.
\textbf{Answer:} Kylie does not have enough money.  \\\cline{2-2}\colorg
  &\colorg \textbf{Table:}  | Price | Quantity demanded | Quantity supplied
| \$165 | 17,900 | 6,400
| \$345 | 15,100 | 8,900
| \$525 | 12,300 | 11,400
| \$705 | 9,500 | 13,900
| \$885 | 6,700 | 16,400
\textbf{Question}: Look at the table. Then answer the question. At a price of \$885, is there a shortage or a surplus?
\textbf{Rationale:}  At the price of \$885, the quantity demanded is less than the quantity supplied. There is too much of the good or service for sale at that price. So, there is a surplus.
\textbf{Answer:} surplus \\\cline{2-2}\colorg
& \colorg\textbf{Table:} | Chickenville | 3:00 A.M. | 12:00 P.M. | 3:30 P.M.
| Floral Gardens | 3:45 A.M. | 12:45 P.M. | 4:15 P.M.
| Pleasant River Campground | 4:45 A.M. | 1:45 P.M. | 5:15 P.M.
| Happy Cow Farm | 5:15 A.M. | 2:15 P.M. | 5:45 P.M.
| Rocky Ravine Town | 5:45 A.M. | 2:45 P.M. | 6:15 P.M.
\textbf{Question}: Look at the following schedule. Doug just missed the 3.00 A.M. train at Chickenville. How long does he have to wait until the next train?
\textbf{Rationale:}  Find 3:00 A. M. in the row for Chickenville. Look for the next train in that row.
The next train is at 12:00 P. M. The elapsed time is 9 hours.
\textbf{Answer:} 9\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\tab{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_tabmwp}
%\vspace{-0.25cm}
\end{table*}



















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS & \textbf{Facts}: Penguins are native to the deep, very cold parts of the southern hemisphere. Miami is located in the northern hemisphere and has a very warm climate.
 \\&\textbf{Question:} Would it be common to find a penguin in Miami?
\\ & \textbf{Rationale:} Where is a typical penguin's natural habitat? What conditions make \#1 suitable for penguins? Are all of \#2 present in Miami?
\textbf{Answer: No}
 \\\cline{2-2}
 & \textbf{Facts:} Shirley Bassey recorded the song Diamonds are Forever in 1971. Over time, diamonds degrade and turn into graphite. Graphite is the same chemical composition found in pencils.
\\ &\textbf{Question:} Is the title of Shirley Bassey's 1971 diamond song a true statement?
 \textbf{Rationale}: What is the title to Shirley Bassey's 1971 diamond song? Do diamonds last for the period in \#1? \textbf{Answer}: No \\\cline{2-2}
 & \textbf{Facts:} The first six numbers in the Fibonacci sequence are 1,1,2,3,5,8. Since 1 is doubled, there are only five different single digit numbers.  \textbf{Question:} Are there five different single-digit Fibonacci numbers?
 \\ &\textbf{Rationale:} What are the single-digit numbers in the Fibonacci sequence? How many unique numbers are in \#1? Does \#2 equal 5?
\textbf{Answer:} Yes\\\cline{2-2}
  & \textbf{Facts:} Katy Perry's gospel album sold about 200 copies. Katy Perry's most recent pop albums sold over 800,000 copies.
\textbf{Question:} Do most fans follow Katy Perry for gospel music?
 \textbf{Rationale:} What type of music is Katy Perry known for? Is Gospel music the same as \#1?
 \textbf{Answer:} No\\\cline{2-2}
    & \textbf{Facts:} The Italian Renaissance was a period of history from the 13th century to 1600. A theocracy is a type of rule in which religious leaders have power. Friar Girolamo Savonarola was the ruler of Florence, after driving out the Medici family, from November 1494 â€ 23 May 1498. \textbf{Question:} Was Florence a Theocracy during Italian Renaissance?
  \textbf{Rationale:} When was the Italian Renaissance?When did Friar Girolamo Savonarola rule Florence? Is \#2 within the span of \#1? Did Friar Girolamo Savonarola belong to a religious order during \#3?
  \textbf{Answer:} Yes\\
  \midrule




  
\colorg \static{} & \colorg \textbf{Facts}: The average cost of a US Boeing 737 plane is 1.6 million dollars. Wonder Woman (2017 film) grossed over 800 million dollars at the box office. \textbf{Question}: Is a Boeing 737 cost covered by Wonder Woman (2017 film) box office receipts?
 \textbf{Rationale:}  How much does a Boeing 737 cost?. How much did the 2017 movie Wonder Woman gross? Is \#2 greater than \#1?
\textbf{Answer:} Yes
 \\\cline{2-2}\colorg
 & \colorg \textbf{Facts}: Big Show is a professional wrestler that weighs 383 pounds. Force is equal to mass times acceleration. An adult Cheetah weighs around 160 pounds. An adult Cheetah can run up to 58 MPH. \textbf{Question:}  Can a cheetah generate enough force to topple Big Show?
\colorg\textbf{Rationale}:  How much does Big Show weigh? How much does a cheetah weigh? How fast can a cheetah run? Is the force produced by a mass of \#2 and a speed of \#3 enough to knock over something that weighs \#1?
 \textbf{Answer}: Yes \\\cline{2-2}\colorg
 & \colorg \textbf{Facts}: Spaghetti and meatballs are a staple on Italian pizzeria menus in the US. The Olive Garden, an Italian family restaurant, has several dishes with meatballs. Meatballs originated in the Chinese Qin dynasty (221 BC to 207 BC). \textbf{Question:} Do restaurants associate meatballs with the wrong country of origin?
 \textbf{Rationale:} In what country is the oldest evidence of people eating meatballs found? What dish involving meatballs became popular in the United States after being invented in New York City in the 20th century? With which national cuisine do Americans typically associate \#2? Are \#3 and \#1 different?
\textbf{Answer:} Yes\\\cline{2-2}\colorg
&\colorg \textbf{Facts:} Torah scrolls must be duplicated precisely by a trained scribe. The Torah has a total of 8,674 words. The population of Bunkie Louisiana is 3,939 people according to a 2018 census. \\ \colorg &\colorg \textbf{Question:} Can you give at least one word from the Torah to all residents of Bunkie Louisiana?
\textbf{Rationale:} How many words are in the Torah? How many residents does Bunkie, Louisiana have? Is \#1 greater than \#2?
\textbf{Answer:} Yes\\\cline{2-2}\colorg
&\colorg \textbf{Facts:} Wrestlemania X took place in 1994. The Toyota Prius was first manufactured in 1997. \textbf{Question:} Could someone have arrived at Wrestlemania X in a Toyota Prius?
\textbf{Rationale:} When did Wrestlemania X hold? When was the Toyota Prius first manufactured? Is \#2 before \#1?
\textbf{Answer:} No\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\strat{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_strategyqa}
%\vspace{-0.25cm}
\end{table*}

==> figures/ablation/sunar_comp_mqa.tex <==

\begin{tikzpicture}
\edef\mylst{"44.58","45.75","54.83"}
\edef\explora{"24.84","0","28.11","32.75","44.28"}

    \begin{axis}[
            ybar=5pt,
            width=4.2cm,
            height=5cm,
            bar width=0.25,
            every axis plot/.append style={fill},
            grid=major,
            xtick={1, 2, 3},
            xticklabels={ PRF, self-ask,\textbf{\name{}}},
            xlabel={},
            ylabel style = {font=\tiny},
        yticklabel style = {font=\boldmath \tiny,xshift=0.05ex},
        xticklabel style ={font=\tiny,yshift=0.5ex},
            ylabel={Task Performance (cover-EM)},
            enlarge x limits=0.25,
            ymin=0,
            ymax=80,
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend cell align={left},
            legend pos=north west,
            legend columns=-1,
    extra y tick style={grid=major,major grid style={thick,draw=black}}, 
            legend style={/tikz/every even column/.append style={column sep=0.5cm}},
        ]
        \addplot+[
            ybar,
            plotColor1*,
            nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\textbf{\mystring},
            nodes near coords align={vertical},
            draw=black,
            postaction={
                    pattern=north east lines
                },
        ] plot coordinates {
                (1,44.58)
                (2,45.75)
                (3,54.83)
            };
            
        \draw[color=black, style=densely dashed,line width = 1.5pt] (axis cs:0,65.55) -- (axis cs:5,65.55)  node[pos=0.2, anchor=west, font=\small, yshift=7pt] {Gold};           
    %     \addplot+[
    %         ybar,
    %         plotColor2*,
    %         draw=black,
    %         nodes near coords=\pgfmathsetmacro{\mystring}{{\explora}[\coordindex]}\textbf{\mystring},
    % nodes near coords align={vertical},
    %         postaction={
    %                 pattern=north west lines
    %             },
    %     ] plot coordinates {
    %             (1,24.84)
    %             (2,0)
    %             (3,28.11)
    %             (4,32.75)
    %             (5,44.28 )
    %         };
 

    \end{axis}


    
\end{tikzpicture}


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \color{purple}
% Is our method specific to in-context numerical reasoning, or can it also work for other NLU tasks? What is special about numerical reasoning? Can we say that we design a general method but test it on numerical reasoning tasks because they are more difficult? \color{green} As semantic similarity between train and test set can't be used to select ICEs in case of numerical reasoning. Therefore we propose EXPLORA.\\
% \color{black}
% \color{blue}
% - We are given only the task-specific loss, which is different from generative model error. We do not utilize the logits given by generative models. Bayesian explanation, in-context one iteration GD -- each of these papers, can we say why these theories don't apply to complex QA.

% Complex numerical reasoning tasks such as financial question answering \cite{chen2022finqa} or tabular question answering \cite{tabmwp} require both language understanding as well as reasoning skills.
% Large language models (LLMs) have been shown to exhibit both these skills.
% Language understanding skills help  While 

% \color{gray}

Answering complex questions that require multi-step numerical reasoning \cite{chen2022finqa,tabmwp,aqua_rat,roy2016solving} over structured and unstructured sources is an active research area with applications in finance, law, and healthcare~\cite{wang2023survey}.
% The complexity in such tasks could arise from multiple factors, such as the need to parse heterogeneous sources like tables and text \cite{chen2022finqa} coupled with multi-step numerical reasoning \cite{tabmwp,aqua_rat,roy2016solving} to answer the question. 

Existing supervised approaches for numerical reasoning involve fine-tuning of multiple generative models for generating arithmetic programs or stepwise solution to the original problem \cite{chiang-chen-2019-semantically,amini-etal-2019-mathqa,aqua_rat,roy2016solving,geva-etal-2020-injecting,cobbe2021training}. 
 
% However, existing approaches require expensive annotations of supervised stepwise rationales along with the solution for fine-tuning multiple generative models \cite{aqua_rat} \cite{cobbe2021training} \cite{geva-etal-2020-injecting} lacking a general purpose solution. 

\begin{figure*}[t]
\centering

\includegraphics[width=0.8\textwidth]{figures/explora-cropped.pdf}\\
\caption{Overview of \static{}, proposed exemplar selection approach.}
\label{fig:icl}
% \vspace{-4mm}
\end{figure*}


More recently, the advances in Large Language Models (LLMs) has lead to substantial progress in a wide range of natural language understanding and reasoning tasks \cite{brown2020gpt3}. The emergent capabilities in LLMs\cite{wei2022emergent,gpt3incontext} such as In-Context Learning (ICL) has paved the way to a new class of approaches that employ chain-of-thought reasoning~\cite{complex_cot} \cite{wei2023chainofthought} for solving complex numerical reasoning questions.
Instead of fine-tuning task-specific models, these approaches focus on choosing carefully constructed exemplars with rationales to be used as input to LLMs, commonly termed as prompting.
% A distinct advantage of prompting with demonstration samples vs fine-tuning is  that the LLM is a general-purpose machine that can be used to solve multiple numerical reasoning tasks.
% In this paper, our focus is to propose a general framework that can be employed to solve multiple QA tasks that require numerical reasoning over homogeneous and heterogeneous sources by selecting suitable demonstration samples.

\mpara{The limitations of manual exemplar selection.} 
% It is inherently hard for the LLMs to perform multi-step reasoning using few-shot in-context learning with just the  \texttt{(input, output)} pairs~\cite{rae2022scaling}.
To tackle complex numerical reasoning problems, \textit{chain-of-thought} (COT) prompting was proposed to add hand-crafted natural language rationales (stepwise solutions) to the prompts in addition to input and output resulting in \texttt{(input, rationale, output)}~\cite{wei2023chainofthought}.
% The process of generating stepwise natural language rationales can be seen as decomposing the original problem to simpler problems that can be solved with less effort \cite{wei2023chainofthought} \cite{brown2020gpt3}.

% Interesting, 
% COT rationales for compositional natural language questions involve generating explanations for the final answer. 
% However, such explanations have been found to be unfaithful to the reasoning process of underlying LLM \cite{turpin2023language,ye2022unreliability} for answering compositional questions in complex QA, unlike numerical reasoning questions. 
% In such cases, the decomposition of such question to simpler sub-questions is observed to be more faithful. To induce such decomposition capabilities in LLMs, authors of the work self-ask \cite{self_ask} modify COT prompting and propose to add hand-crafted follow-up questions derived from the original complex questions to the prompt.
However, there are inherent limitations of COT approach for complex and hybrid numerical reasoning tasks. 
The COT involves the manual effort of selecting the best exemplars with appropriate rationales that sufficiently convey the  execution strategy for the task under consideration. The manual selection process is tedious and not scalable across different numerical reasoning tasks. Since the outputs generated by the LLM are highly sensitive to exemplars provided \cite{lu-etal-2022-fantastically,zhao2021calibrate,chang2023data}, it is crucial to select meaningful exemplars that are robust across evaluation samples and improve overall task performance.

\mpara{Limitations of automated exemplar selection approaches}:
To tackle these limitations, several automated exemplar selection approaches have been proposed \cite{ye2023compositional,lu-etal-2022-fantastically,rubin-etal-2022-learning,complex_cot}. These approaches are usually dynamic exemplar selection methods, which select several demonstration examples from the training set for each test example. Several approaches also require annotated data and training of several models for exemplar selection\cite{lu2023dynamic,ye2023compositional}. These approaches entail to heavy computational requirements during inference, especially when there is a large pool of exemplars to select from. While unsupervised approaches like similarity \cite{rubin-etal-2022-learning} or diversity based \cite{ye-etal-2023-complementary} approaches exist for dynamic exemplar selection, they also require projecting the input query and the entire pool of exemplars to a continuous vector space followed by search, increasing computational time during inference. Additionally, the majority of these approaches assume the exemplars chosen to be independent of each other and only consider the interaction between the test sample and the exemplars. They do not account for the interactions between the exemplars themselves.

 As an alternative to dynamic exemplar selection approaches, LENS \cite{li2023finding} proposed to select a static set of task level support exemplars. However, LENS assumes access to language model output logits and involves multiple expensive evaluations of the LLM for scoring the exemplars. LENS also does not model the interactions between exemplars and scores each sample independently. 
% In the example below, using Few-shot-COT results in inaccurate results due to lack of decomposition information in its prompt (hidden due to space reasons).
% \input{intro-example-mouth}

\mpara{\static{} (Static Exemplar Selection Approach):}
In this work, we propose a novel static exemplar selection method \static{}, that selects multiple high value/low loss exemplar subsets. An overview of the working of \static{} is shown in Figure \ref{fig:icl}. The selection of task level exemplar subsets are performed once, and we model the interactions between exemplars through initial sampling of subsets and by directly scoring and selecting subsets. We propose a parameterized scoring function that approximates the loss indicative of task performance using features from a transformer based embedding model. We propose an exploration mechanism as shown in Figure \ref{fig:icl} to estimate the parameters of the scoring function with minimal calls to the LLM and without access to logits from the LLM. Our approach mitigates the expensive processing during inference incurred by traditional dynamic exemplar selection approaches and obviates the need for manual exemplar selection while providing high performance.


\mpara{Contributions.} The core contributions of our work are:
\begin{description}
    \item 
    1) We propose a new robust static exemplar selection approach \static{}, that selects task level exemplars for numerical reasoning based questions.

    \item 
    2) We demonstrate the ability of transferring selected exemplars across models. We show that exemplars selected using smaller models can be used to induce reasoning capabilities in much larger models leading to reduced costs.
     \item 
     3) We demonstrate that \static{} is less resource intensive compared to existing approaches, as it results in minimal calls to the LLMs for exemplar selection.
    \item 
    4) We conduct extensive experiments with different exemplar selection methods to showcase the generalized performance of \static{} across multiple complex and hybrid numerical reasoning based QA tasks.
\end{description}

\color{black}


==> llama3.1_results.tex <==
\begin{table*}[ht]
\centering

\renewcommand{\arraystretch}{1.3} % Increase row height
\begin{tabular}{lccccc}
\toprule
\textbf{Model}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Temporal Overlap} & \textbf{Time Jaccard} \\
\midrule
\rowcolor[gray]{0.93} \multicolumn{6}{l}{\textbf{Closed Book}} \\

\textbf{Meta Llama 3.1} & & & & & \\
\fshot{} & 0.48 & 0.376 & 0.397 & 0.466 & 0.398 \\ 
\knn{} \fshot{} & 0.464 & 0.415 & 0.414 & 0.495 & 0.421 \\
\COT{} & 0.511 & 0.399 & 0.412 & 0.578 & 0.446 \\ 
Auto COT{} & 0.381 & 0.302 & 0.31 & 0.439 & 0.356 \\ 

\rowcolor[gray]{0.93} \multicolumn{6}{l}{\textbf{Open Book}} \\
\textbf{BM25} & 0.606 & 0.530 & 0.540 & 0.658 & 0.603 \\
\textbf{all-minim-v2} & 0.444 & 0.389 & 0.393 & 0.479 & 0.425  \\
\textbf{multi-qa-mpnet} & 0.416 & 0.340 & 0.353 & 0.468 & 0.379 \\

\rowcolor[gray]{0.93} \multicolumn{6}{l}{\textbf{Golden Evidence}} \\
\textbf{Meta Llama 3.1} & & & & & \\
\fshot{} & 0.922 & 0.837 & 0.866 & 0.880 & 0.861 \\ 
\knn{} \fshot{} & 0.928 & 0.886 & 0.899 & 0.940 & 0.925 \\ 
\bottomrule
\end{tabular}
\caption{Performance of various models on the benchmark using different prompting techniques (Llama 3.1)}
\label{tab:llama_3_1}
\end{table*}


==> manual-cot-prompt.tex <==
\begin{table}[htb!!]
\begin{tcolorbox}[title=Prompt: Manual Chain of Thought]
\small
\textbf{\ding{228} \textsc{System Message}}: You are tasked with providing rationale and answers to timeline-based queries about various subjects. \newline
Your reply should be structured in this format: \texttt{Rationale: \{your rationale\} /n Final answer: \{your answer\}} \vspace{0.2cm}

Each answer should be structured as a list, with different entries for each subject or title. Each entry must include the years corresponding to the following the title or subject. \vspace{0.2cm}

Please adhere to the following structure in your responses: \\
- Write the title or name first, exactly as it would appear in a formal context such as Wikipedia. \\
- Follow the title or name with a colon and then the years. \\
- Represent a range of years by using a short dash. \\
- Separate multiple years or ranges with a comma and a space. \\
- End each entry with a comma, except for the last entry. \\
- If the current year is relevant to the query, use "2024" instead of "present". \\
- Each answer should be on a new line, with no additional characters or explanations. \\
- Ensure the completeness and correctness of your answers. Try to be as complete as possible. \\
- If provided examples, follow the example structure and reasoning style. \vspace{0.2cm}

\textbf{\ding{228} \textsc{User Message (Example)}}: \textit{List all political positions Greg Abbott held to this day.} \\ \vspace{0.2cm}

\textbf{\ding{228} \textsc{Assistant Message (Example)}}: \newline 
\texttt{Rationale}: \textit{Greg Abbott is an American politician and officeholder. He was first known to be the Justice of the Supreme Court in Texas. He started in 1996 and resigned in 2001. In 2002, he got elected as the 50th Attorney General of Texas. In 2014, Abbott announced his candidacy for Governor of Texas. He won the elections and became Governor of Texas in 2015. To this day, he still holds this office. Between 2019 and 2020, he was also the Chair of the Republican Governors Association.} \newline
\texttt{Final answer:} \newline
\textit{"Governor of Texas": 2015-2024,} \newline
\textit{"Chair of the Republican Governors Association": 2019-2020,} \newline
\textit{"50th Attorney General of Texas": 2002-2015,} \newline
\textit{"Justice of the Supreme Court of Texas": 1996-2001} \\ \vspace{0.2cm}

\textbf{\ding{228} \textsc{User Message}}: \textit{List all political positions Brian Pallister held to this day.} \vspace{0.2cm} \\ 

\end{tcolorbox}
\captionof{figure}{Manual COT prompt setup (closed book setting)}
\label{fig:rationale_prompt}
\end{table}


==> ndcg_plots.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ndcg_plot.png}
    \caption{Comparison of retrieval models (nDCG) }
                \label{fig:retriever_extra_2}

\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/recall_plot.png}
    \caption{Comparison of retrieval models (Recall) }
                \label{fig:retriever_extra_1}

\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/precision_plot.png}
    \caption{Comparison of retrieval models (Precision). }
        \label{fig:retriever_extra}
\end{figure}

==> prompt-aqua.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= AQUA Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math. Follow given examples and solve the problems in step by step manner.}



\paragraph{\textbf{Exemplars}}:

[Question]: \textit{ The average age of three boys is 45 years and their ages are in proportion 3:5:7. What is the age in years of the youngest boy?}

[Options]: A) 9, B) 10, C) 11, D) 12, E) 13

[Explanation]: \textsf{$3x + 5x + 7x = 45$, \\ $x =3$, \\ $3x = 9$}

[Answer]: \textcolor{teal}{\textsf{The option is A}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Question: {}
Options: {}

Explanation: [INS]
Answer: [INS]

\end{tcolorbox}
\captionof{figure}{Prompt for \aqua{}}
\label{prompt:aqua} 
\end{table*}

==> prompt-finqa.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= FinQA Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math, using the information from given table and text.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





\textit{Read the following table, and then answer the question:}

[Table]: Year | 2016 | 2015 | 2014 |\\
share-based compensation expense | $30809$ | $21056$ | $29793$ | \\
income tax benefit | $9879$ | $6907$ | $7126$ |

[Question]: \textit{how much percent did the income tax benefit increase from 2014 to 2016?}

[Explanation]: \textsf{$x0=( 9879 - 7126$ ), \\ ans=( $x0 / 7126$ )}

[Answer]: \textcolor{teal}{\textsf{The answer is increased 38.6\%}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
Table: {}
Question: {}

Explanation: [INS]
Answer: [INS]




\end{tcolorbox}
\captionof{figure}{Prompt for \fin{}}
\label{prompt:finqa} 
\end{table*}

==> prompt-tabmwp.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= TabMWP Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math, using the information from the given table. Solve the given problem step by step providing an explanation for your answer.}



\paragraph{\textbf{Exemplars}}:

[Table]: Table: Day | Number of tickets \\
Monday | $36$ \\
Tuesday | $43$ \\
Wednesday | $46$ \\
Thursday | $59$ \\
Friday | $37$ \\
Saturday | $46$ \\
Sunday | $51$ 


[Question]: \textit{The transportation company tracked the number of train tickets sold in the past 7 days. What is the range of the numbers?}

[Explanation]: \textsf{Read the numbers from the table. $36$, $43$, $46$, $59$, $37$, $46$, $51$ \\ First, find the greatest number. The greatest number is $59$. \\ Next, find the least number. The least number is $36$. \\ Subtract the least number from the greatest number: $59$ - $36$ = $23$}

[Answer]: \textcolor{teal}{\textsf{The range is 23}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Table: {}
Question: {}

Explanation: [INS]
Answer: [INS]




\end{tcolorbox}
\captionof{figure}{Prompt for \tab{}}
\label{prompt:tabmwp} 
\end{table*}

==> prompt_gsm8k.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= GSM8K Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math. Follow given examples and solve the problems in step by step manner.}



\paragraph{\textbf{Exemplars}}:

[Question]: \textit{Samir just turned half the age Hania was $10$ years ago. If in five years Hania will be $45$ years old, what will Samir's age be five years from now?}

[Explanation]: \textsf{If in five years, Hania will be $45$ years old, currently she is $45-5 = 40$ years old.\\
Samir just turned half the age Hania was $10$ years ago, which means she is $30/2 = 15$ years old. \\
In five years, Samir will be $15+5 = 20$ years old.}

[Answer]: \textcolor{teal}{\textsf{20 years old}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Question: {}

Explanation: [INS]
Answer: [INS]

\end{tcolorbox}
\captionof{figure}{Prompt for \gsm{}}
\label{prompt:gsm8k} 
\end{table*}


==> prompt_strategy.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= StrategyQA Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve commonsense problems requiring reasoning. Follow the given examples that use the facts to answer a question by decomposing into sub-questions first and then predicting the final answer as "Yes" or "No" only.}



\paragraph{\textbf{Exemplars}}:

[Facts]: Snowden scored above $145$ on two separate IQ tests. The minimum accepted IQ score for MENSA on the Stanford–Binet is $132$, while for the Cattell it is $148$.

[Question]: \textit{Could Edward Snowden join MENSA?}

[Sub-question 1]: \textsf{What is the minimum accepted IQ score to be admitted to MENSA?\\}
[Sub-question 2]: \textsf{What is Edward Snowden's IQ?\\}
[Sub-question 3]: \textsf{Is \#2 greater than or equal to \#1?}


[Answer]: \textcolor{teal}{\textsf{Yes}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Facts: {} Question: {}

Sub-question: [INS]
Answer: [INS]

\end{tcolorbox}
\captionof{figure}{Prompt for \strat{}}
\label{prompt:strategy} 
\end{table*}


==> prompts/prompt_decomp.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= DecomP Prompt]
\small
\textbf{Instruction}:\texttt{Solve a question answering task with interleaving retrieval 
Follow the given examples and Given the question and context, use relevant evidence for each subquestion from given list of evidences, answer the subquestion and output final answer for the question using information in the context, answers to subquestions and give final answer strictly preceded by  [Final Answer]:}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138  100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





[Question]: In which country did this Australian who was detained in Guantanamo Bay detention camp
and published Guantanamo: My Journey receive para-military training?


Subquestion 1: (select) [retrieve odqa] Who is the Australian who was detained in Guantanamo Bay detention
camp and published ”Guantanamo: My Journey”?


Answer: {”titles”: [”Guantanamo: My Journey”, ”Bismullah v. Gates”, ”Guantanamo Bay detention
camp”], ”answer”: [”David Hicks”]}


Subquestion 1: (select) [retrieve odqa] In which country did David Hicks receive his para-military training?


Answer: {”titles”: [”John Adams Project”, ”Camp Echo (Guantanamo Bay)”, ”Guantanamo Bay
Museum of Art and History”, ”David Hicks”], ”answer”: [”Afghanistan”]}


Subquestion 3: (select) [multihop titleqa] Titles: [”Guantanamo: My Journey”, ”Bismullah v. Gates”, ”
Guantanamo Bay detention camp”, ”John Adams Project”, ”Camp Echo (Guantanamo Bay)”,
”Guantanamo Bay Museum of Art and History”, ”David Hicks”]. 

Question: In which country
did this Australian who was detained in Guantanamo Bay detention camp and published ``
Guantanamo My Journey" receive para-military training?


[Final Answer]: Afghanistan
\\



[Question]: who is older Jeremy Horn or Renato Sobral ?
Subquestion 1: (select) [retrieve odqa] When was Jeremy Horn born?


Answer: {”titles”: [”Zaza Tkeshelashvili”, ”Jeremy Horn”, ”Jeremy Horn (singer)”, ”Ricardo Arona”], ”
answer”: [”August 25, 1975”]}


Subquestion 2: (select) [retrieve odqa] When was Renato Sobral born?


Answer: {”titles”: [”Brian Warren”, ”Renato Sobral”], ”answer”: [”September 7, 1975”]}


Subquestion 3: (select) [multihop titleqa] Titles: [”Zaza Tkeshelashvili”, ”Jeremy Horn”, ”Jeremy Horn (
singer)”, ”Ricardo Arona”, ”Brian Warren”, ”Renato Sobral”]. Question: who is older Jeremy
Horn or Renato Sobral ?


[Final Answer]: Jeremy Horn
\\

[Question]: What was the 2014 population of the city where Lake Wales Medical Center is located?

Subquestion 1: (select) [retrieve odqa] Lake Wales Medical Center is located in what city?

Answer: {”titles”: [”Baylor College of Medicine”, ”Lake Wales Medical Center”, ”Tufts University
School of Medicine”, ”Hanford Community Medical Center”], ”answer”: [”Polk County,
Florida”]}

Subquestion 2: (select) [retrieve odqa] What was the population of Polk County in 2014?

Answer: {”titles”: [”Banner University Medical Center Tucson”, ”Lake Wales, Florida”], ”answer”:
[”15,140”]}

Subquestion 3: (select) [multihop titleqa] Titles: [”Baylor College of Medicine”, ”Lake Wales Medical Center
”, ”Tufts University School of Medicine”, ”Hanford Community Medical Center”, ”Banner
University Medical Center Tucson”, ”Lake Wales, Florida”]. Question: What was the 2014
population of the city where Lake Wales Medical Center is located?

[Final Answer]: 15,140
\\


[Question]: Nobody Loves You was written by John Lennon and released on what album that was issued
by Apple Records, and was written, recorded, and released during his 18 month separation
from Yoko Ono?

Subquestion 1: (select) [retrieve odqa] What album was issued by Apple Records, and written, recorded, and
released during John Lennon’s 18 month separation from Yoko Ono?

Answer: {”titles”: [”John Lennon/Plastic Ono Band”, ”Milk and Honey (album)”, ”Walls and Bridges”],
”answer”: [”Walls and Bridges”]}

Subquestion 2: (select) [retrieve odqa] Nobody Loves You was written by John Lennon on what album?

Answer: {”titles”: [”John Lennon Museum”, ”Nobody Loves You (When You’re Down and Out)”], ”
answer”: [”Walls and Bridges”]}

Subquestion 3: (select) [multihop titleqa] Titles: [”John Lennon/Plastic Ono Band”, ”Milk and Honey (album)

[Final Answer]: Walls and Bridges
                      [\dots]


\paragraph{\textbf{Input}:} "Follow the above examples, and use the given Evidence: "+\{\}+"  and use the information from the evidence to answer the original question  and give final answer strictly preceded by [Final Answer]: for the   Question: \{\}


\end{tcolorbox}
\captionof{figure}{DeComP prompt \cite{khot2023decomposed}}
\label{prompt:decomp} 
\end{table*}



==> prompts/prompt_meta_reasoner.tex <==
\begin{table}[hbt!]

\begin{tcolorbox}[title= Meta-Reasoner Prompt]
\small
\textbf{Instruction}:\texttt{Follow the given examples and Given the question and context, reasoning path, think step by step extract key segments from given evidence relevant to question and give rationale, by forming your own reasoning path preceded by [Answer]: and output final answer for the question using information from given evidences and give concise precise answer preceded by [Final Answer]:.}



\paragraph{\textbf{Exemplars}}: \{\} \\

Given the above examples and 
\\\textbf{Existing reasoner path}: \{Reasoning path from $\name{}_R$\}, \\
\textbf{the evidence} : \{top-$l$ evidences across sub-questions\} \\ and use the most relevant information for the question from the most relevant evidence from given Evidence: and form your own correct reasoning path to derive the answer thinking step by step preceded by [Answer]: and subsequently give final answer as shown in above examples preceded by [Final Answer]: for \\ \textbf{the Question}: \{Test Question\}

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





\end{tcolorbox}
\captionof{figure}{Meta-reasoner prompt}
\label{fig:meta} 
\end{table}



==> prompts/prompt_react.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= ReAct Prompt]
\small
\textbf{Instruction}:\texttt{Solve a question answering task with interleaving Thought, Action, Observation steps. Thought can reason about the current situation, and Action can be three types: 
(1) Search[entity], which searches the exact entity on Wikipedia and returns the first paragraph if it exists. If not, it will return some similar entities to search.
(2) Lookup[keyword], which returns the next sentence containing keyword in the current passage.
(3) Finish[answer], which returns the answer and finishes the task.:}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: What is the elevation range for the area that the eastern sector of the Colorado orogeny extends into?\\
                Thought 1: I need to search Colorado orogeny, find the area that the eastern sector of the Colorado orogeny extends into, then find the elevation range of the area.\\
                Action 1: Search[Colorado orogeny]\\
                Observation 1: The Colorado orogeny was an episode of mountain building (an orogeny) in Colorado and surrounding areas.\\
                Thought 2: It does not mention the eastern sector. So I need to look up eastern sector.\\
                Action 2: Lookup[eastern sector]\\
                Observation 2: (Result 1 / 1) The eastern sector extends into the High Plains and is called the Central Plains orogeny.\\
                Thought 3: The eastern sector of Colorado orogeny extends into the High Plains. So I need to search High Plains and find its elevation range.\\
                Action 3: Search[High Plains]\\
                Observation 3: High Plains refers to one of two distinct land regions:\\
                Thought 4: I need to instead search High Plains (United States).\\
                Action 4: Search[High Plains (United States)]\\
                Observation 4: The High Plains are a subregion of the Great Plains. From east to west, the High Plains rise in elevation from around 1,800 to 7,000 ft (550 to 2,130 m).[3]\\
                Thought 5: High Plains rise in elevation from around 1,800 to 7,000 ft, so the answer is 1,800 to 7,000 ft.\\
                Action 5: Finish[1,800 to 7,000 ft]

                
                [Final Answer]: 1,800 to 7,000 ft \\
                Question: Musician and satirist Allie Goertz wrote a song about the \"The Simpsons\" character Milhouse, who Matt Groening named after who?\\
                Thought 1: The question simplifies to \"The Simpsons\" character Milhouse is named after who. I only need to search Milhouse and find who it is named after.\\
                Action 1: Search[Milhouse]\\
                Observation 1: Milhouse Mussolini Van Houten is a recurring character in the Fox animated television series The Simpsons voiced by Pamela Hayden and created by Matt Groening.\\
                Thought 2: The paragraph does not tell who Milhouse is named after, maybe I can look up \"named after\".\\
                Action 2: Lookup[named after]\\Observation 2: (Result 1 / 1) Milhouse was named after U.S. president Richard Nixon, whose middle name was Milhous. \\
                Thought 3: Milhouse was named after U.S. president Richard Nixon, so the answer is Richard Nixon.\\
                Action 3: Finish[Richard Nixon]\\Question: Which documentary is about Finnish rock groups, Adam Clayton Powell or The Saimaa Gesture?\\
                Thought 1: I need to search Adam Clayton Powell and The Saimaa Gesture, and find which documentary is about Finnish rock groups.\\
                Action 1: Search[Adam Clayton Powell]\\
                Observation 1: Could not find [Adam Clayton Powell]. Similar: ['Adam Clayton Powell III', 'Seventh Avenue (Manhattan)', 'Adam Clayton Powell Jr. State Office Building', 'Isabel Washington Powell', 'Adam Powell', 'Adam Clayton Powell (film)', 'Giancarlo Esposito'].\\
                Thought 2: To find the documentary, I can search Adam Clayton Powell (film).\\
                Action 2: Search[Adam Clayton Powell (film)]\\
                Observation 2: Adam Clayton Powell is a 1989 American documentary film directed by Richard Kilberg.\\
                The film is about the rise and fall of influential African-American politician Adam Clayton Powell Jr.[3][4] It was later aired as part of the PBS series The American Experience.\\
                Thought 3: Adam Clayton Powell (film) is a documentary about an African-American politician, not Finnish rock groups. So the documentary about Finnish rock groups must instead be The Saimaa Gesture.\\
                Action 3: Finish[The Saimaa Gesture]

                
                [Final Answer]: The Saimaa Gesture \\

  
[\dots]

\paragraph{\textbf{Input}:} "Follow the above examples, and use the given Evidence: "+\{\}+" \\ and use the information from the evidence to answer the original question  and give final answer strictly preceded by [Final Answer]: for the   Question: \{\}
\end{tcolorbox}
\captionof{figure}{ReAct prompt \cite{khot2023decomposed}}
\label{prompt:react} 
\end{table*}



==> prompts/prompt_searchain.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= SearChain Prompt]
\small
\textbf{Instruction}:\texttt{Solve a question answering task with interleaving Thought, Action, Observation steps. Thought can reason about the current situation, and Action can be three types: 
(1) Search[entity], which searches the exact entity on Wikipedia and returns the first paragraph if it exists. If not, it will return some similar entities to search. \\
(2) Lookup[keyword], which returns the next sentence containing keyword in the current passage. \\
(3) Finish[answer], which returns the answer and finishes the task.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: When does monsoon season end in the state the area code 575 is located? \\
Are follow up questions needed here: Yes. \\
Follow up: Which state is the area code 575 located in?\\
Intermediate Answer: The area code 575 is located in New Mexico. \\
Follow up: When does monsoon season end in New Mexico? \\
Intermediate Answer: Monsoon season in New Mexico typically ends in mid-September. 

[Final Answer]: mid-September. 
\\


Construct a global reasoning chain for this complex [Question] : " \{\} " You should generate a query to the search engine based on
        what you already know at each step of the reasoning chain, starting with [Query]. \\
                        If you know the answer for [Query], generate it starting with [Answer]. \\
                        You can try to generate the final answer for the [Question] by referring to the [Query]-[Answer] pairs, starting with [Final
                        Answer].\\
                        If you don't know the answer, generate a query to search engine based on what you already know and do not know, starting with
                        [Unsolved Query]. \\
                        For example:
                        [Question]: "Where do greyhound buses that are in the birthplace of Spirit If...'s performer leave from? "

                        
                        [Query 1]: Who is the performer of Spirit If... ? \\
                        If you don't know the answer: 

                        
                        [Unsolved Query]: Who is the performer of Spirit If... ? \\
                        If you know the answer:
                        [Answer 1]: The performer of Spirit If... is Kevin Drew.
                        [Query 2]: Where was Kevin Drew born? \\
                        If you don't know the answer:
                        [Unsolved Query]: Where was Kevin Drew born? \\
                        If you know the answer:
                        [Answer 2]: Toronto. 
                        
                        [Query 3]: Where do greyhound buses in Toronto leave from? \\
                        If you don't know the answer:
                        [Unsolved Query]: Where do greyhound buses in Toronto leave from? \\
                        If you know the answer:
                        [Answer 3]: Toronto Coach Terminal. 
                        
                        [Final Content]: The performer of Spirit If... is Kevin Drew [1]. Kevin Drew was born in Toronto [2]. Greyhound buses in
                        Toronto leave from Toronto
                        Coach Terminal [3]. So the final answer is Toronto Coach Terminal. 
                        
                        [Final Answer]: Toronto Coach Terminal 

                        
                        [Question]:"Which magazine was started first Arthur’s Magazine or First for Women?" 

                        
                        [Query 1]: When was Arthur’s Magazine started? 

                        
                        [Answer 1]: 1844. 

                        
                        [Query 2]: When was First for Women started?
                        [Answer 2]: 1989 

                        
                        [Final Content]: Arthur’s Magazine started in 1844 [1]. First for Women started in 1989 [2]. So Arthur’s Magazine was started
                        first. So the answer is Arthur’s Magazi 
                        

                        
                        [Final Answer]: Arthur’s Magazi.
                      [\dots]




\end{tcolorbox}
\captionof{figure}{Searchain prompt used for complex QA \cite{xu2024searchinthechaininteractivelyenhancinglarge}}
\label{prompt:searchain} 
\end{table*}



==> prompts/self_ask_prompt.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= \self{} 2WikiMultiHopQA Prompt]
\small
\textbf{Instruction}:\texttt{Follow the given examples and Given the question determine if followup questions are needed and decompose the original question.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: Who lived longer, Theodor Haecker or Harry Vaughan Watkins? \\
                Are follow up questions needed here: Yes.\\
Follow up: How old was Theodor Haecker when he died?\\
Intermediate Answer: Theodor Haecker was 65 years old when he died.\\
Follow up: How old was Harry Vaughan Watkins when he died?\\
Intermediate Answer: Harry Vaughan Watkins was 69 years old when he died.

[Final Answer]: Harry Vaughan Watkins.
\\
Question: Why did the founder of Versus die? \\
Are follow up questions needed here: Yes.\\
Follow up: Who founded Versus?\\
Intermediate Answer: Gianni Versace.\\
Follow up: Why did Gianni Versace die?\\
Intermediate Answer: Gianni Versace was shot and killed on the steps of his Miami Beach mansion on July 15, 1997.
[Final Answer]: Shot.
\\
Question: Who is the grandchild of Dambar Shah? \\
Are follow up questions needed here: Yes. \\
Follow up: Who is the child of Dambar Shah? \\
Intermediate Answer: Dambar Shah (? - 1645) was the king of the Gorkha Kingdom. He was the father of Krishna Shah. \\
Follow up: Who is the child of Krishna Shah? \\
Intermediate Answer: Krishna Shah (? - 1661) was the king of the Gorkha Kingdom. He was the father of Rudra Shah. 
[Final Answer]: Rudra Shah.
\\
Question: Are both director of film FAQ: Frequently Asked Questions and director of film The Big Money from the same
country? \\
Are follow up questions needed here: Yes. \\
Follow up: Who directed the film FAQ: Frequently Asked Questions?\\
Intermediate Answer: Carlos Atanes.\\
Follow up: Who directed the film The Big Money?
Intermediate Answer: John Paddy Carstairs.
Follow up: What is the nationality of Carlos Atanes?
Intermediate Answer: Carlos Atanes is Spanish.
Follow up: What is the nationality of John Paddy Carstairs?\\
Intermediate Answer: John Paddy Carstairs is British.
[Final Answer]: No.
\\
Question: Who was the maternal grandfather of George Washington? \\
Are follow up questions needed here: Yes.
Follow up: Who was the mother of George Washington?\\
Intermediate answer: The mother of George Washington was Mary Ball Washington. \\
Follow up: Who was the father of Mary Ball Washington? \\
Intermediate answer: The father of Mary Ball Washington was Joseph Ball.
[Final Answer]: Joseph Ball 
\\


\paragraph{\textbf{Input}}: Based on above examples, given the Question: {} determine, Are followup questions needed here ?




\end{tcolorbox}
\captionof{figure}{Example of In-context learning for 2WikiMultiHopQA through \self{} based prompting of LLMs }
\label{prompt:wqa} 
\end{table*}



==> prompts/self_ask_prompt_mqa.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= \self{} MusiqueQA Prompt]
\small
\textbf{Instruction}:\texttt{Follow the given examples and Given the question determine if followup questions are needed and decompose the original question.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





Question: When does monsoon season end in the state the area code 575 is located? \\
Are follow up questions needed here: Yes. \\
Follow up: Which state is the area code 575 located in?\\
Intermediate Answer: The area code 575 is located in New Mexico. \\
Follow up: When does monsoon season end in New Mexico? \\
Intermediate Answer: Monsoon season in New Mexico typically ends in mid-September. 

[Final Answer]: mid-September. 
\\


Question: What is the current official currency in the country where Ineabelle Diaz is a citizen? \\
Are follow up questions needed here: Yes. \\
Follow up: Which country is Ineabelle Diaz a citizen of? \\
Intermediate Answer: Ineabelle Diaz is from Peurto Rico, which is in the United States of America. \\
Follow up: What is the current official currency in the United States of America? \\
Intermediate Answer: The current official currency in the United States is the United States dollar.
[Final Answer]: United States dollar.
\\

Question: Where was the person who founded the American Institute of Public Opinion in 1935 born?
Are follow up questions needed here: Yes.
Follow up: Who founded the American Institute of Public Opinion in 1935?
Intermediate Answer: George Gallup.
Follow up: Where was George Gallup born?
Intermediate Answer: George Gallup was born in Jefferson, Iowa.

[Final Answer]: Jefferson.
\\


Question: What is the sports team the person played for who scored the first touchdown in Superbowl 1?  \\
Are follow up questions needed here: Yes. \\
Follow up: Which player scored the first touchdown in Superbowl 1? \\
Intermediate Answer: Max McGee. \\
Follow up: Which sports team did Max McGee play for? \\
Intermediate Answer: Max McGee played for the Green Bay Packers.

[Final Answer]: Green Bay Packers.
\\

Question: The birth country of Jayantha Ketagoda left the British Empire when? \\
Are follow up questions needed here: Yes. \\
Follow up: What is the birth country of Jayantha Ketagoda? \\
Intermediate Answer: Sri Lanka. \\
Follow up: When did Sri Lanka leave the British Empire? \\
Intermediate Answer: Sri Lanka left the British Empire on February 4, 1948. 

[Final Answer]: February 4, 1948 \\
                      
\paragraph{\textbf{Input}}: Based on above examples, given the Question: {} determine, Are followup questions needed here ?




\end{tcolorbox}
\captionof{figure}{Example of In-context learning for MusiqueQA (MQA) through \self{} based prompting of LLMs}
\label{prompt:mqa} 
\end{table*}



==> qualitative_analysis.tex <==
\begin{table*}[t!]
\centering
 % \scalebox{0.8}{
% \begin{tabular}{p{2cm}p{1.3cm}p{1.3cm}p{1.3cm}}

\begin{tabular}{lccc}
\hline
\textbf{GAC}  ($\kappa$)& \textbf{GEU} ($\kappa_K$) & \textbf{AC} ($\kappa$) & \textbf{EU} ($\kappa$)\\ 
\hline

\midrule
 4.87$\pm$0.32 (0.77) & 4.93$\pm$0.24 (0.64)& 3.65$\pm$1.37 (0.86) & 3.35$\pm$1.68 (0.79) \\

% \numdecomp{}  & 0.779 & \textbf{0.581} \\
 
\bottomrule
\end{tabular}
% }
\caption{Manual evaluation. AC: Answer Completeness, EU : Evidence usefulness, G indicates Ground Truth. We use the Likert scale (1-5) and Cohen's Kappa ($\kappa$) for inter-annotator agreement (in brackets).}
\label{tab:question_quality}
\end{table*}



==> rag-prompt.tex <==
\begin{table}[htb!!]
\begin{tcolorbox}[title=Prompt: Retrieval Augmented Generation]
\small
\textbf{\ding{228} \textsc{System Message}}: You are tasked with responding to timeline-based queries about various subjects. \newline
Each response should be structured as a list, with different entries for each subject or title. Each entry must include the years corresponding to the title or subject. \newline
You will receive additional context from the user regarding the query. Use the context as additional sources to answer the query. \vspace{0.2cm}

Please adhere to the following structure in your responses: \\
- Write the title or name first, exactly as it would appear in a formal context such as Wikipedia. \\
- Follow the title or name with a colon and then the years. \\
- Represent a range of years by using a short dash. \\
- Separate multiple years or ranges with a comma and a space. \\
- End each entry with a comma, except for the last entry. \\
- If the current year is relevant to the query, use "2024" instead of "present". \\
- Each answer should be on a new line, with no additional characters or explanations. \\
- Ensure the completeness and correctness of your answers. \vspace{0.2cm}

\textbf{Example response format:} \\
\texttt{Title or Name: year1-year2, year3} \\
\texttt{Title or Name: Years}, \vspace{0.2cm}

% Show User Message and some context
\textbf{\ding{228} \textsc{User Message (Example)}}: \textit{List all political positions Joe Biden held to this day.} \vspace{0.2cm} \\
\textbf{Context:} \newline
\textit{Infobox: \newline
Order: 46th \newline
Office: President of the United States \newline
Vicepresident: Kamala Harris \newline
Term Start: January 20, 2021 \newline
Predecessor: Donald Trump \newline
... \newline
Other offices: \newline
Chair of the International Narcotics Control Caucus (2007–2009) \newline
Chair of the Senate Foreign Relations Committee (2001–2003, 2007–2009) \newline
Chair of the Senate Judiciary Committee (1987–1995) \newline
Member of the New Castle County Council (1971–1973)
} \\ \vspace{0.2cm}

% Assistant Message generated based on context
\textbf{\ding{228} \textsc{Assistant Message (Example)}}: \newline 
\textit{President of the United States (2021-2024)} \newline
\textit{Vice President of the United States (2009-2017)} \newline
\textit{United States Senator from Delaware (1973-2009)} \\ \vspace{0.2cm}

% New user message
\textbf{\ding{228} \textsc{User Message}}: \textit{List all political positions Brian Pallister held to this day.} \vspace{0.2cm} \\ 

\end{tcolorbox}
\captionof{figure}{RAG prompt (open book and golden evidence)}
\label{fig:timeline_query_response}
\end{table}


==> table-datasets.tex <==
\begin{table*}[b]
\resizebox{\textwidth}{!}{

\begin{tabular}{lccll}

\hline
\textbf{Dataset} & \textbf{\#Train} & \textbf{\#Test} & \textbf{Example Question} & \textbf{Description} \\ \hline



\colorg    & \colorg   & \colorg     & \colorg \texttt{Claire makes a 3 egg omelet every morning}      & multi-step  \colorg   \\
\colorg \textbf{GSM8K}~\cite{cobbe2021training}& \colorg 7473 & \colorg 1319 & \colorg  \texttt{for breakfast. How many dozens of eggs will}  & arithmetic word  \colorg    \\
\colorg & \colorg & \colorg & \colorg \texttt{she eat in 4 weeks?} & problems \colorg  \\


 &    &   &  \texttt{A trader sold an article at a profit of 20\%}      &   multi-step  \\
\textbf{AquaRat}~\cite{aqua_rat}& 97467 & 254 &  \texttt{for Rs.360. What is the cost price of the} & arithmetic word  \\
&  & & \texttt{article?} & problems  \\



\colorg   & \colorg    & \colorg   & \colorg  \texttt{Allie kept track of how many kilometers she}      & \colorg Table based   \\
\colorg \textbf{TabMWP}~\cite{tabmwp} & \colorg 23059 & \colorg 7686 & \colorg  \texttt{walked during the past 5 days. What is the} &\colorg numerical     \\
\colorg & \colorg & \colorg  & \colorg \texttt{range of the numbers?} &\colorg reasoning \\


 &    &   & \texttt{In 2010 and 2009, what was total fair value}      & Table and Text  \\
\textbf{FinQA}~\cite{chen2022finqa} & 6251 & 1147 & \texttt{in billions of assets segregated for benefit}      & based numerical  \\
& & & \texttt{of securities and futures brokerage customers?}      & reasoning
\\


\colorg   & \colorg    & \colorg   & \colorg  \texttt{Would the chef at Carmine's restaurant panic}      & \colorg multi-step   \\
\colorg \textbf{StrategyQA}~\cite{geva2021did} & \colorg 1800 & \colorg 490 & \colorg  \texttt{if there was no basil?} &\colorg reasoning     \\



\bottomrule
\end{tabular}
}
\caption{Overview of the Complex QA datasets used in this study.}
\label{tab:datasets_overview}
\end{table*}

==> table-qualitative.tex <==



\begin{table*}
\begin{tabular}{lp{.80\textwidth}}
\toprule
    \textbf{Method}     & \textbf{Decomposition} \\
\midrule


\colorg \textbf{Question}  & \colorg \textbf{In 2010 and 2009 , what was the total fair value in billions of assets segregated for the benefit of securities and futures brokerage customers?} [Dataset: \textbf{FinQA}] \\
\COT{}  & To find the total fair value in billions of assets segregated for the benefit of securities and futures brokerage customers in 2010 and 2009, we need to look at the table. \textcolor{red}{In 2010, the fair value was \$25.0 billion and in 2009, it was \$24.0 billion. Hence total is \textbf{Answer:} \$49 billion.}  \\
\colorg \icat{} + \ftd{} & \colorg \textbf{Rationale:} To find the total fair value in billions [\dots], look at the table for the years 2010 and 2009. In the table, under "year ended December 31," we can see two columns [\dots], there is a row labeled "securities and futures brokerage customers." In this row, there are values listed in millions.To convert these values to billions, we divide each value by 1000.
\textcolor{teal}{For 2010: \$25.0 billion (segregated cash) + \$9.7 billion (fair value of securities) = \$34.7 billion
For 2009: \$24.0 billion (segregated cash) + \$10.2 billion (fair value of securities) = \$34.2 billion
[\dots] \textbf{Answer:} 68.9}
 \\
\icat{} & in billions, we need to look at Note 29 in the text. 
In 2010, \$25.0 billion in cash and \$9.7 billion in securities with [\dots]. 
In 2009, \$24.0 billion in cash and \$10.2 billion in securities [\dots].
\textbf{Answer}: \texttt{68.9 (billion)}. \\
\midrule
\midrule


\end{tabular}
\caption{Qualitative analysis of reasoning chains generated by chain-of-thought vs \icat{}}
\label{tab:qualitative}
%\vspace{-0.25cm}
\end{table*}



==> table-result-exhaustive-evaluation.tex <==

\begin{table}[!t]
    \footnotesize
    \centering
     \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccc}
    \toprule
    \small

\textbf{Datasets} & \textbf{GSM} & \textbf{Aqua} & \textbf{Tab} & \textbf{Fin} & \textbf{Strat}\\


    
    \midrule

    Exhaustive eval &76.72   &50.39   &  82.24 &  57.02 & 82.45\\

    \static{} (-exploration) & 75.89& 50.00& 75.16 & 50.30 & 80.40\\
    \ \hspace{4em} (Mistral) & \\
    
    \textbf{\static{}(Llama)} & \textbf{79.07}  & \textbf{53.94}  & 80.11  &  54.66 & \textbf{85.31} \\

    \textbf{\static{}(Mistral)} & \textbf{77.86}  & \textbf{53.54}  & \textbf{83.07}  &  \textbf{59.46} & \textbf{85.71} \\
    
      \bottomrule
    \end{tabular}
    } 
    \caption{Ablation studies: exhaustive evaluation, w/o exploration vs proposed exploration (\static{}).}
    % \vspace{-1cm}
    \label{tab:exhaustive_evaluation}
\end{table}


==> table-results-SOTA.tex <==
\begin{table*}[t]
    \footnotesize
    \small

    \centering

     \resizebox{\textwidth}{!}{%
    \begin{tabular}{llllll}

    \toprule
     \textbf{Method}& \multicolumn{1}{l}{\textbf{GSM8K}}& \multicolumn{1}{l}{\textbf{AquaRat}} & \multicolumn{1}{l}{\textbf{TabMWP}} & \multicolumn{1}{l}{\textbf{FinQA}} 
     & \multicolumn{1}{l}{\textbf{StrategyQA}}  
     \\
     
    %     \midrule
    
    % SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
    \midrule
    % \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\
       \colorg \textbf{dynamic} & \colorg & \colorg & \colorg & \colorg & \colorg \\
    KNN  \cite{rubin-etal-2022-learning}              &53.45    &51.96    &77.07   &51.52  & 81.83    \\
        KNN (S-BERT)  \cite{rubin-etal-2022-learning}              &53.07    &52.75    &77.95   &52.65  & 81.83    \\
    MMR  \cite{ye-etal-2023-complementary}            &54.36    &51.18    &77.32   &49.87    & 82.86  \\
    KNN+SC \cite{wang2022self}                        &80.21    &62.59    &83.08   &54.49 & 83.88     \\
    MMR+SC \cite{wang2022self}                        &78.01    &59.45    &81.36   &50.74  & 83.88    \\
    PromptPG \cite{lu2023dynamic}                     & \centering -       & -       &68.23   &53.56  & -    \\
    % \color{red}DQ-LoRe \color{black} \cite{xiong2023dq} & \centering -       & -       &-   &-  & -    \\


    \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg & \colorg \\
    Zero-Shot COT \cite{kojima2023large}              &67.02    &49.60    &57.10   &47.51 & 59.75         \\
    Manual Few-Shot COT \cite{wei2023chainofthought}  &73.46    &44.88    &71.22   &52.22 & 73.06     \\
    Random                                            &67.79    &49.80    &55.89   &53.70 &  81.02     \\
    PS+ \cite{wang-etal-2023-plan}                    &59.30    &46.00    & -      & -   & -      \\
    Auto-COT \cite{zhang2023automatic}                &57.10    &41.70    & -      & -  & 71.20       \\
    GraphCut \cite{iyer2013submodular}                &66.19    &47.24    &60.45   &52.31 & 80.00    \\ 
    FacilityLocation \cite{iyer2013submodular}        &68.61    &48.43    &67.66   &36.79 &  81.63    \\ 
    LENS \cite{li2023finding}                         &69.37    &48.82    &77.27  &54.75  & 79.79    \\ 
    LENS+SC \cite{li2023finding}                         &79.37    & 57.87   &  80.68 & 60.06   & 82.24  \\ 

     \colorg \textbf{Our Approach} & \colorg& \colorg& \colorg& \colorg & \colorg\\
     
    \textbf{\static{}}                 &\colorit 77.86\up{12.24} $\dagger$ &\colorit 53.54\up{9.67}$\dagger$ &\colorit 83.07\up{7.51} $\dagger$ &\colorit 59.46\up{8.60} $\dagger$ &\colorit 85.71\up{5.63} $\dagger$\\
    
    \textbf{\static{}+\selfcon{}}      &\textbf{86.35}\up{24.48} $\ddagger$&63.39\up{29.84} $\ddagger$  &85.52\up{10.68} $\ddagger$   &64.52\up{17.84}  $\ddagger$ & 87.14 \up{9.21}$\dagger$   \\
    
    \textbf{\static{}+\knn+\selfcon{}} &85.14 \up{22.73}$\ddagger$  & 62.20\up{27.41}$\ddagger$ & 86.29\up{12.39} $\ddagger$  &\textbf{65.12}\up{18.94}  $\ddagger$ & \textbf{88.37}\up{10.75}$\dagger$   \\
    
    \textbf{\static{}+\mmr+\selfcon{}} &86.13\up{24.16} $\ddagger$ &\textbf{63.78}\up{30.64} $\ddagger$&\textbf{86.96}\up{12.54}$\ddagger$    &64.60\up{17.99}   $\ddagger$    & 87.55\up{9.73}$\dagger$       \\


  
    
%     \midrule
%     \colorg \textbf{Mistral} & \colorg& \colorg& \colorg& \colorg\\
% %     \colorg \textbf{dynamic} & \colorg& \colorg& \colorg& \colorg\\
% % KNN                         &37.98  &23.22 &61.74 &9.06   \\ 
% %     KNN+SC                      &61.71  &35.02 &67.98 &11.33  \\
% %     MMR                         &46.25  &18.11 &52.82 &10.11  \\
% %     MMR+SC                      &62.24  &33.07 &65.08 &12.03  \\
% %         \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg\\
%     Zero-Shot COT               &7.43   &      &43.34 &       \\
%     Few Shot COT                &30.48  &14.90 &46.94 &       \\
%     Random                      &33.81  &22.04 &30.40 &5.52   \\ 
%     LENS                        &       &      &      &       \\ 
    
%     \static{}                   &45.41  &30.07 &48.79 &5.57   \\
%     \static{}+\selfcon{}        &61.41  &34.10 &61.96 &7.41   \\
%     \static{}+\knn+\selfcon{}   &62.92  &23.22 &59.91 &4.79   \\
%     \static{}+\mmr+\selfcon{}   &60.05  &22.44 &61.29 &5.40   \\
%     \static{}+\pot{}+\selfcon{} &56.33  &26.00 &61.24 &10.11  \\

%     \midrule
%     \colorg \textbf{Llama-2-7B} & \colorg& \colorg& \colorg& \colorg\\

%     %     \colorg \textbf{dynamic} & \colorg& \colorg& \colorg& \colorg\\
%     % KNN                         &23.43  &28.34 &54.83 &10.37  \\
%     % KNN+SC                      &39.80  &34.8  &64.18 &11.33  \\
%     % MMR                         &29.64  &21.65 &49.61 &12.20  \\
%     % MMR+SC                      &38.74  &27.16 &56.99 &12.90  \\
%     %       \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg\\ 
%     Zero-Shot COT               &6.14   &      &40.31 &       \\
%     Few Shot COT                &21.15  &20.47 &43.23 &       \\
%     Random                      &18.27  &21.6  &28.41 &4.62   \\ 
%     LENS                        &       &      &      &       \\ 

%     \static{}                   &27.67  &24.40 &46.25 &6.62   \\
%     \static{}+\selfcon{}        &36.85  &24.01 &56.74 &6.21   \\
%     \static{}+\knn+\selfcon{}   &38.21  &22.83 &49.80 &5.92   \\
%     \static{}+\mmr+\selfcon{}   &38.60  &26.77 &51.68 &6.36   \\
%     \static{}+\pot{}+\selfcon{} &23.35  &      &45.44 &10.28  \\
%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    % random &  20.28& 25.33&  81.71 & 74.7  \\
    
    % \mmr+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    % \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    % \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


%         \midrule
%  \colorg \textbf{Mistral} & \colorg& \colorg& \colorg& \colorg\\
  
%     random &  20.28& 25.33&  81.71 & 74.7  \\
    
%     \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
%     \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
%     \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


%       \midrule
% \colorg \textbf{Llama-2-7B} &\colorg & \colorg& \colorg& \colorg\\

%    random&  24.36& 29.41&  92.95 &   77.60  \\

%     \mmr+\selfcon{}  &  26.99& 30.69&  \coloritt  95.13 & \colorit  80.70  \\
    
%      \static{}+\selfcon{}  &  27.07& 30.33&  94.96 & \colorit  80.70  \\
     
%     \static{}+\pot{}+\selfcon{} &  \coloritt  \textbf{27.24}$\ddagger$& \coloritt  \textbf{36.00}&  \colorit  \textbf{96.14}$\dagger$ & \colorit  \textbf{80.70}  \\



 %        \midrule
 % \colorg \textbf{FLAN-T5-XL} & \colorg& \colorg& \colorg& \colorg\\
  
 %    random &  20.28& 25.33&  81.71 & 74.7  \\
    
 %    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
 %    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
 %    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\
     
     \bottomrule
    \end{tabular}
    } 
    \caption{Results across datasets using gpt-3.5-turbo model as backbone. Percentage improvements are reported over LENS \cite{li2023finding}.  $\dagger$ indicates statistical significance using t-test over LENS at 0.05 level and $\ddagger$  at 0.01 level.}
    % \vspace{-1cm}
    \label{tab:main_result}
\end{table*}

% \color{purple} SB: Can we split this table into two - first one with only GPT3 results claiming state of the art performance (add a lot more baseline results), and second one improvement over other exemplar selection techniques ?






==> table-results-llm-calls.tex <==
\begin{table*}[t]
    \centering
    % resizebox{\textwidth}{!}{% 
    \begin{tabular}{lccccccc}
    \toprule

\textbf{Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ COT\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Few-Shot\\  COT\end{tabular}} & \textbf{Random} & \textbf{KNN}  & \textbf{MMR}  & \textbf{LENS} & \textbf{Explora} \\
    
     % \textbf{Datasets}& \multicolumn{1}{c}{\textbf{Zero-Shot COT}}& \multicolumn{1}{c}{\textbf{Few-shot COT}} & \multicolumn{1}{c}{\textbf{Random}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{LENS}} & \multicolumn{1}{c}{\textbf{Explora}}  \\
    

    \midrule

    \textbf{GSM8K}    &1319   &1319   &1319   &1319    &1319    &24176     &4719   \\
    \textbf{AquaRat}  &254    &254    &254    &254     &254     &23111     &3654   \\
    \textbf{TabMWP}   &7686   &7686   &7686   &7686    &7686    &30543     &11086  \\
    \textbf{FinQA}    &1147   &1147   &1147   &1147    &1147    &24004     &4547   \\
      \bottomrule
    \end{tabular}
    % } 
    \caption{Frugal subset selection approach - we reduce number of calls to LLMs. Our score based approach enables us to make fewer calls to LLMs compared to LENS which lacks this score based modelling.}
    % \vspace{-1cm}
    \label{tab:llm_calls}
\end{table*}


==> table-results-llms_transfer.tex <==
\begin{table}[!t]
\footnotesize
    \centering
    \small
     \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\textbf{T}} & \multicolumn{1}{c}{\textbf{GSM}}& \multicolumn{1}{c}{\textbf{Aqua}} & \multicolumn{1}{c}{\textbf{Tab}} & \multicolumn{1}{c}{\textbf{Fin}}
     & \multicolumn{1}{c}{\textbf{Strat}} \\
     

    %     \midrule
    
    % SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
    \midrule
    % \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\

    \textbf{\staticshort{}}                &  L    &79.07  &53.94  & 80.11     &  54.66  & 85.31    \\
                             &  M   &77.86  &53.54  & 83.07     &  59.46 & 85.71    \\
    \textbf{\staticshort{}+\selfcon{}}     &  L    &85.82  &63.78  & 86.76     &  61.16  & 85.10   \\
                             &  M   &86.35  &63.39  & 85.52     &  64.52  & 87.14    \\
    \textbf{\staticshort{}+\knn+\selfcon{}}&  L    &85.89  &64.17  & 85.74     &  63.64  & 86.53   \\
                             &  M   &85.14  &62.20  & 86.29     &  65.12 & 88.37    \\
    \textbf{\staticshort{}+\mmr+\selfcon{}}&  L    &86.20  &62.99  & 87.81     &  64.60  & 86.12   \\
                             &  M   &86.13  &63.78  & 86.96     &  64.60   & 87.55  \\



     \bottomrule
    \end{tabular}
    } 
    \caption{Results for transfer (T) of exemplars selected using \static{} (\staticshort{}) on smaller LLMs (Llama2-7b (L) and Mistral-7b (M)) to larger LLM (gpt-3.5-turbo).}
    % \vspace{-1cm}
    \label{tab:llm_transfer}
\end{table}








==> table-results-robustness.tex <==
% \begin{table*}[t]
%     \footnotesize
%     \centering
%     % resizebox{\textwidth}{!}{% 
%     \begin{tabular}{lccccccccc}
%     \toprule

% \textbf{Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ COT\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Few-Shot\\  COT\end{tabular}}  & \textbf{KNN}  & \textbf{MMR}  & \textbf{\begin{tabular}[c]{@{}c@{}}Graph \\ Cut\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Facility \\ Location\end{tabular}}  & \textbf{LENS} & \textbf{Explora} \\
    
%      % \textbf{Datasets}& \multicolumn{1}{c}{\textbf{Zero-Shot COT}}& \multicolumn{1}{c}{\textbf{Few-shot COT}} & \multicolumn{1}{c}{\textbf{Random}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{LENS}} & \multicolumn{1}{c}{\textbf{Explora}}  \\
    

%     \midrule

%     \textbf{GSM8K}    & $\pm$5.18   & $\pm$4.48     &  $\pm$3.76 & $\pm$4.00   & $\pm$6.38  &  $\pm$4.23&  $\pm$5.04     & \textbf{$\pm$3.39}  \\
%     \textbf{AquaRat}  & $\pm$7.08  &  $\pm$12.03 & $\pm$5.49  &  $\pm$10.53  &  $\pm$8.18  & $\pm$6.71  & $\pm$6.67 & \textbf{$\pm$4.93}  \\
%     \textbf{TabMWP}   & $\pm$1.84   & $\pm$1.66  &  $\pm$1.27 &  $\pm$1.68  & $\pm$2.03   &  $\pm$1.74    & $\pm$1.72 & $\pm$1.45 \\
%     \textbf{FinQA}    & $\pm$4.50  & $\pm$4.76  & $\pm$4.17  &  $\pm$6.10  & $\pm$5.29   &  $\pm$4.94 &  $\pm$5.81 & \textbf{$\pm$3.41}  \\
%       \bottomrule
%     \end{tabular}
%     % } 
%     \caption{Comparison of robustness of \static{} to other approaches. We report standard deviation (lower is better) using scores from different splits of test set.}
%     % \vspace{-1cm}
%     \label{tab:robustness}
% \end{table*}













\begin{table}[!t]
    \footnotesize
    \centering
     \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccc}
    \toprule
    \small

\textbf{Datasets} & \textbf{GSM} & \textbf{Aqua} & \textbf{Tab} & \textbf{Fin} & \textbf{Strat}\\

% \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ COT\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Few-Shot\\  COT\end{tabular}}  & \textbf{KNN}  & \textbf{MMR}  & \textbf{\begin{tabular}[c]{@{}c@{}}Graph \\ Cut\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Facility \\ Location\end{tabular}}  & \textbf{LENS} & \textbf{Explora} \\
    
    \midrule

    Zero-Shot COT    & $\pm$5.18   & $\pm$7.08     &  $\pm$1.84 & $\pm$4.50 & $\pm$4.19     \\
    Few-Shot COT  & $\pm$4.48  &  $\pm$12.03 & $\pm$1.66  &  $\pm$4.76 & $\pm$5.67   \\
    KNN   & $\pm$3.76   & $\pm$5.49  &  $\pm$1.27 &  $\pm$4.17  & $\pm$4.85 \\
    MMR    & $\pm$4.00  & $\pm$10.53  & $\pm$1.68  &  $\pm$6.10 &  $\pm$5.70  \\
    Graph Cut & $\pm$6.38& $\pm$8.18  & $\pm$2.03  &  $\pm$5.29 & $\pm$7.62 \\
    Facility Location & $\pm$4.23  & $\pm$6.71  & $\pm$1.74  &  $\pm$4.94 & $\pm$5.93 \\
    LENS & $\pm$5.04  & $\pm$6.67  & $\pm$1.59  &  $\pm$5.81 & $\pm$ 3.98 \\
    \textbf{\static{}} & $\pm$\textbf{3.39}  & $\pm$\textbf{4.93}  & $\pm$1.50  &  $\pm$\textbf{3.41} &$\pm$ \textbf{3.95} \\
    
      \bottomrule
    \end{tabular}
    } 
    \caption{Comparison of robustness of \static{} to other approaches. We report standard deviation (lower is better) with scores from different splits of eval. set.}
    % \vspace{-1cm}
    \label{tab:robustness}
\end{table}


==> table-results-small-models.tex <==
\begin{table*}[hbt!]
    \centering
    % resizebox{\textwidth}{!}{% 
    \begin{tabular}{lcccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\textbf{GSM8K}}& \multicolumn{1}{c}{\textbf{AquaRat}} & \multicolumn{1}{c}{\textbf{TabMWP}} & \multicolumn{1}{c}{\textbf{FinQA}} \\
     

    %     \midrule
    
    % SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
    \midrule
    \colorg \textbf{Mistral-7B} & \colorg& \colorg& \colorg & \colorg \\\\
       \colorg \textbf{dynamic} & \colorg & \colorg & \colorg & \colorg   \\
    KNN  \cite{rubin-etal-2022-learning}             &37.98  &23.22    &61.74   & 9.06       \\
    MMR  \cite{ye-etal-2023-complementary}           &46.25  &18.11    &52.82   & 10.11      \\
    % KNN+SC \cite{wang2022self}                       &61.71  &35.02    &67.98   & 11.33      \\
    % MMR+SC \cite{wang2022self}                       &62.24  &33.07    &65.08   & 12.03      \\
    % PromptPG \cite{lu2023dynamic}                  & -     & -       & 68.23  & 53.56      \\


    \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg\\
    Zero-Shot COT \cite{kojima2023large}             &7.43   &21.65    &43.34   &1.74        \\
    Manual Few-shot COT \cite{wei2023chainofthought} &30.48  &14.90    &46.94   &3.22        \\
    Random                                           &33.81  &22.04    &30.40   &5.52        \\
    % PS+ \cite{wang-etal-2023-plan}                 &59.30  &46.00    & -      & -          \\
    % Auto-COT \cite{zhang2023automatic}             &57.10  &41.70    & -      & -          \\
    GraphCut \cite{iyer2013submodular}               &47.00  &21.65    &59.46   &5.66        \\ 
    FacilityLocation \cite{iyer2013submodular}       &46.25  &14.17    &57.74   &4.96        \\ 
    LENS \cite{li2023finding}                        &46.39  &29.92    &57.69   &5.14        \\ 


    \colorg \textbf{Our Approach} & \colorg& \colorg& \colorg& \colorg \\
    \static{}                                        & 46.41  &30.07    &58.62   &5.57        \\
    \static{}+\selfcon{}                     &\textbf{61.41}  &\textbf{35.10}   &\textbf{61.96}   &7.41        \\
    % \static{}+\knn+\selfcon{}               &\textbf{62.92}  &23.22    &59.91   &4.79        \\
    % \static{}+\mmr+\selfcon{}                        &60.05  &22.44    &61.29   &5.40        \\
    % \static{}+\pot{}+\selfcon{} &76.87  &      &      &   \\



\midrule
    \colorg \textbf{Llama2-7B} & \colorg& \colorg& \colorg& \colorg \\\\
       \colorg \textbf{dynamic} & \colorg & \colorg & \colorg & \colorg  \\
    KNN  \cite{rubin-etal-2022-learning}             &23.43  &28.34    &54.83   & 10.37      \\
    MMR  \cite{ye-etal-2023-complementary}           &29.64  &21.65    &49.61   & 12.20      \\
    % KNN+SC \cite{wang2022self}                       &38.80  &34.80    &64.18   & 11.33      \\
    % MMR+SC \cite{wang2022self}                       &38.74  &27.16    &56.99   & 12.90      \\
    % PromptPG \cite{lu2023dynamic}                  & -     & -       & 68.23  & 53.56      \\


    \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg \\
    Zero-Shot COT \cite{kojima2023large}             &6.14   &6.29     &40.31   &1.67        \\
    Manual Few-shot COT \cite{wei2023chainofthought} &21.15  &20.47    &43.23   &2.87        \\
    Random                                           &18.27  &21.60    &28.41   &4.62        \\
    % PS+ \cite{wang-etal-2023-plan}                 &59.30  &46.00    & -      & -          \\
    % Auto-COT \cite{zhang2023automatic}             &57.10  &41.70    & -      & -          \\
    GraphCut \cite{iyer2013submodular}               &27.29  &21.65    &47.38   &5.40        \\ 
    FacilityLocation \cite{iyer2013submodular}       &27.21  &21.65    &47.23   &5.05        \\ 
    LENS \cite{li2023finding}                        &28.05  &23.22    &48.29   &6.62        \\ 


    \colorg \textbf{Our Approach} & \colorg& \colorg& \colorg& \colorg \\
    \static{}                                        &28.67  &24.40    &49.96   &6.62        \\
    \static{}+\selfcon{}                             &\textbf{36.85}  &24.01    & \textbf{56.74}  &6.21        \\
    % \static{}+\knn+\selfcon{}                        &38.21  &22.83    &49.80   &5.92        \\
    % \static{}+\mmr+\selfcon{}               &\textbf{38.90}  &26.77    &51.68   &6.36        \\
    % \static{}+\pot{}+\selfcon{} &76.87  &      &      &   \\

  
    
     \bottomrule
    \end{tabular}
    % } 
    \caption{Results across datasets on \mistral{} and \llamaseven{}.}
    % \vspace{-1cm}
    \label{tab:main_result_small_models}
\end{table*}








==> table-results-v2.tex <==
\begin{table*}[!t]
    \centering
    
    \begin{tabular}{lcccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\aqua{}}& \multicolumn{1}{c}{\strat{}} & \multicolumn{1}{c}{\advhotpot{}} & \multicolumn{1}{c}{\tab{}}  \\
     
     % & cover-EM & cover-EM& EM& EM&EM \\
    %  \midrule
    %  \fshot{}& 11.66& 28.41& 85.74& 78.2& 42.55\\
     
    %  \COT{} &20.85& 34.08&94.79&  79.4&52.22 \\
     
    %  \zfshot{} & 12.22& 19.25& 88.75& 75.4& 47.51 \\
    % \hline
    % \self{} & 23.64& 32.58& N/A& N/A& N/A \\
      
    %   \autocot{} &  N/A& N/A&  93.83 & 76.2 & N/A \\

        \midrule
    
    SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
        \midrule
 \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


        \midrule
 \colorg \textbf{Mistral} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


      \midrule
\colorg \textbf{Llama-2-7B} &\colorg & \colorg& \colorg& \colorg\\

   random&  24.36& 29.41&  92.95 &   77.60  \\

    \mmr+\selfcon{}  &  26.99& 30.69&  \coloritt  95.13 & \colorit  80.70  \\
    
     \static{}+\selfcon{}  &  27.07& 30.33&  94.96 & \colorit  80.70  \\
     
    \static{}+\pot{}+\selfcon{} &  \coloritt  \textbf{27.24}$\ddagger$& \coloritt  \textbf{36.00}&  \colorit  \textbf{96.14}$\dagger$ & \colorit  \textbf{80.70}  \\



        \midrule
 \colorg \textbf{FLAN-T5-XL} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\
     
     \bottomrule
    \end{tabular}
    \caption{Results across datasets. $\dagger$ and $\ddagger$ indicates statistical significance over \COT{} at 0.1 level  and 0.01 level respectively. SOTA results are included for completion.}
    % \vspace{-1cm}
    \label{tab:main_result}
\end{table*}


==> table_category_perf.tex <==
\begin{table*}[ht]
\centering

\renewcommand{\arraystretch}{1.3} % Increase row height
\begin{tabular}{llcccccc}
\toprule
\textbf{Model} & \textbf{Type} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{Temporal Overlap}} & \multicolumn{1}{c}{\textbf{Time Jaccard}} \\
\midrule
\multicolumn{7}{>{\columncolor[gray]{0.93}}l}{\textbf{Closed Book}} \\
\multirow{2}{*}{Mistral KNN} & Sports & 0.469 & 0.245 & 0.308 & 0.420 & 0.322 \\
 & Political & 0.593 & 0.374 & 0.423 & 0.459 & 0.402 \\
\multirow{2}{*}{Meta Llama KNN} & Sports & 0.512 & 0.357 & 0.408 & 0.467 & 0.358 \\
 & Political & 0.583 & 0.440 & 0.477 & 0.568 & 0.493 \\

\multicolumn{7}{>{\columncolor[gray]{0.93}}l}{\textbf{Open Book}} \\
\multirow{2}{*}{Mistral BM25} & Sports & 0.800 & 0.545 & 0.630 & 0.730 & 0.675 \\
 & Political & 0.690 & 0.606 & 0.619 & 0.571 & 0.535 \\
\multirow{2}{*}{Mistral all-mini-lm} & Sports & 0.516 & 0.294 & 0.358 & 0.419 & 0.350 \\
 & Political & 0.628 & 0.463 & 0.503 & 0.424 & 0.393 \\
\multirow{2}{*}{Mistral Multi QA} & Sports & 0.517 & 0.312 & 0.373 & 0.433 & 0.348 \\
 & Political & 0.634 & 0.474 & 0.511 & 0.445 & 0.411 \\

\multicolumn{7}{>{\columncolor[gray]{0.93}}l}{\textbf{Golden Evidence}} \\
\multirow{2}{*}{Mistral Golden Manual} & Sports & 0.941 & 0.661 & 0.763 & 0.862 & 0.818 \\
 & Political & 0.898 & 0.876 & 0.874 & 0.634 & 0.613 \\
\multirow{2}{*}{Mistral Golden KNN} & Sports & 0.935 & 0.760 & 0.828 & 0.897 & 0.847 \\
 & Political & 0.949 & 0.940 & 0.935 & 0.816 & 0.792 \\
\bottomrule
\end{tabular}
\caption{Performance of various models on the benchmark using different prompting techniques, categorized by question type (Sports and Political) using Mistral v0.2}
\label{tab:sports_vs_political_performance}
\end{table*}

==> tables/decomposed_retrieval.tex <==
\begin{table}[h!]
\small
\centering
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{p{2.8cm}cccc}
\toprule
\multirow{2}{*}{\textbf{Retriever}}  & \multicolumn{2}{c}{\textbf{MQA}} & \multicolumn{2}{c}{\textbf{WQA}}  \\
\cmidrule{2-5}
 & R@1 & R@10 &R@1 & R@10 \\
\midrule
\multirow{1}{*}{\self(Re-Rank)} &  0.157 & 0.309  & 0.230   & 0.402   \\
 %SPLADEV2+re-rank &  & &0.294 &0.210 \\
\self{}(Retrieval) & 0.152 & 0.240& 0.205& 0.399 \\
%PRF (re-retrieval) & & & \\
$ \name{}$ & \textbf{0.284}& \textbf{0.459}& \textbf{0.287} & \textbf{0.606} \\
%  \name{} & & & \textbf{} & \textbf{} \\

\bottomrule
\end{tabular}
\caption{Retrieval performances on MQA and WQA  with query understanding. }
\label{table:decomposed_comparison_retrieval}
\end{table}

==> tables/fig-nar-overview.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/sunar-v2.pdf}
    \caption{Overview of \name{} with Neighborhood Aware Retrieval (NAR) and LLM based feedback.}
    \label{fig:main}
\end{figure*}

==> tables/retrieval_comparison.tex <==
\begin{table}[h!]
\small
\centering
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{p{2.8cm}cccc}
\toprule
\multirow{2}{*}{\textbf{Retriever}}  & \multicolumn{2}{c}{\textbf{MQA}} & \multicolumn{2}{c}{\textbf{WQA}}  \\
\cmidrule{2-5}
 & nDCG & R@10 &nDCG & R@10 \\
\midrule
\multirow{1}{*}{SPLADEV2} &  0.155 & 0.062  & 0.251   & 0.186   \\
 %SPLADEV2+re-rank &  & &0.294 &0.210 \\
PRF & 0.183 & 0.065& 0.271& 0.190 \\
%PRF (re-retrieval) & & & \\
$ \name{}_{R}$ & 0.179& \textbf{0.073}& \textbf{0.297} & \textbf{0.216} \\
%  \name{} & & & \textbf{} & \textbf{} \\

\bottomrule
\end{tabular}
\caption{Retrieval performances on MQA and WQA  w/o query understanding. }
\label{table:comparison_retrieval}
\end{table}


==> tables/retrieval_performance.tex <==
\begin{table}[h!]
\small
\centering
\begin{tabular}{p{1.2cm}cccc}
\toprule
\multirow{2}{*}{\textbf{Retriever}}  & \multicolumn{2}{c}{\textbf{MQA}} & \multicolumn{2}{c}{\textbf{WQA}}  \\
\cmidrule{2-5}
 & nDCG & R@100 &nDCG@10 & R@100 \\
\midrule
\multirow{1}{*}{SPLADeV2} &  \textbf{0.155} & \textbf{0.181} & \textbf{0.251}   & \textbf{0.323}   \\
\midrule
\multirow{1}{*}{DPR} & 0.109 & 0.107  & 0.126 & 0.179  \\
\multirow{1}{*}{ANCE} & 0.140 & 0.115 & 0.212 & 0.223   \\

\midrule
\multirow{1}{*}{Tas-b} & 0.176 & 0.172 & 0.277 & 0.303 \\
\multirow{1}{*}{MPNet} & 0.163  & 0.149 & 0.222 & 0.253  \\
\multirow{1}{*}{Contriever} &  0.155 & 0.169 & 0.216 & 0.294   \\
\bottomrule
\end{tabular}
\caption{Performance of different retrieval models on MQA and WQA when documents are retrieved using original question.}
\label{table:retrieval_performance}
\end{table}


==> tables/reward_model.tex <==
\begin{table*}[htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Per Class F1}} & \multicolumn{2}{c}{\textbf{Overall F1 Score}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-6}
& \textbf{T-F1} & \textbf{F-F1} & \textbf{C-F1} & \textbf{Macro} & \textbf{Weighted} \\
\midrule
\textbf{Llama-3.1 8B} \\
% \multicolumn{6}{l}{\textbf{Majority voting}} \\
% \midrule

Top 1 Decoding & 33.5  & 66.4 & 34.7   & 44.8  & 52.5 \\

Self-Consistency \cite{self_consistency} & 
34.9 & 
68.6 & 
35.1 & 
46.2 & 
54.2 \\

Best of N (\name{}) & 
\textbf{44.2} (\textcolor{darkgreen}{+31.9\%}) & 
\textbf{75.3} (\textcolor{darkgreen}{+13.4\%}) & 
\textbf{40.3} (\textcolor{darkgreen}{+16.1\%}) & 
\textbf{53.2} (\textcolor{darkgreen}{+18.8\%}) & 
\textbf{61.0} (\textcolor{darkgreen}{+16.2\%}) \\

Theoretical upper bound & 63.9  & 85.1 & 69.6   & 72.9  & 77.4 \\
\midrule
\textbf{Gpt-4o-mini} \\
Top 1 decoding & 40.68 & 63.14 & 37.99 &47.27 & 52.84 \\
Self-Consistency \cite{self_consistency} & 29.70 & 63.20 & 42.33 & 45.07 & 51.83 \\
Best of N (\name{}) & &   \\
Theoretical upper bound & 45.34 & 85.37 & 67.19 & 65.97 & 73.41 \\

\bottomrule
\end{tabular}}

\captionsetup{font=small}
\caption{Reasoning performance of the models. Here the number of samples for majority voting and best of N sampling is set to 10. The generator model is llama-3.1-Instruct-8b, and the reward model is fine-tuned llama-3.2-3b. The gains method is computed w.r.t the \textit{top 1 Decoding} baseline.}
\label{tab:rm_performance_table}
\end{table*}

==> tables/sunar_ablations.tex <==
\begin{table}[!t]
    \centering
    \small
    \begin{tabular}{lccc}
    \toprule
     \textbf{Method}& \multicolumn{1}{c}{MQA}& \multicolumn{1}{c}{\wqa{}}\\

     % & cover-EM & cover-EM& EM& EM&EM \\
     \midrule
          % \colorg \textbf{gpt-40-mini} & \colorg& \colorg& \colorg\\
     \name{} & \textbf{32.75} & \textbf{54.83} \\
    \name{} (-ASU) & 30.43& 50.75 \\
    % \name{}_{R} (-MER) & & \\

        $\name{}_{R}$ (-ASU) (-MER) & 28.11 & 47.67 \\


     %          \colorg \textbf{Llama 3.2} & \colorg& \colorg& \colorg\\

     %    \self{} & & \\
     % \name{} & & \\

     %               \colorg \textbf{Mistral v0.2} & \colorg& \colorg& \colorg\\

     %    \self{}
     % \name{} & & \\
     
     \bottomrule
    \end{tabular}
    \caption{Ablations of \name{} (gpt-3.5-turbo).}
    \label{tab:ablations}
\end{table}


==> tables/table-llm-substrates.tex <==
\begin{table}[!t]
    \centering
    \small
    \begin{tabular}{lccc}
    \toprule
     \textbf{Method}& \multicolumn{1}{c}{MQA}& \multicolumn{1}{c}{\wqa{}}\\

     % & cover-EM & cover-EM& EM& EM&EM \\
     \midrule
          \colorg \textbf{gpt-4o-mini} & \colorg& \colorg& \colorg\\

        \self{} & 26.76  & 37.33 \\
     \name{} & \textbf{32.19} & \textbf{48.16} \\

              \colorg \textbf{Llama 3.1 (8B)} & \colorg& \colorg& \colorg\\

        \self{} & 5.43& 25.83 \\
     \name{} & \textbf{13.82} & \textbf{39.52} \\

                   \colorg \textbf{Mistral v0.2 (7B)} & \colorg& \colorg& \colorg\\

        \self{} & 7.84 & 27.72\\
     \name{} & \textbf{26.12}& \textbf{40.23}\\
     
     \bottomrule
    \end{tabular}
    \caption{Results across different LLM substrates.}
    \label{tab:llm_substrates}
\end{table}


==> tables/table-ranking.tex <==
\begin{table}[!t]
    \centering
    \small
    \setlength{\tabcolsep}{2.0pt}
    \begin{tabular}{lccc}
    \toprule
     \textbf{Method}& \multicolumn{1}{c}{MQA}& \multicolumn{1}{c}{\wqa{}}\\

     % & cover-EM & cover-EM& EM& EM&EM \\
     \midrule

              \colorg \textbf{Methods (w/ query understanding)} & \colorg& \colorg& \colorg\\
    %\self{} \cite{self_ask} & 15.00& 32.92 \\

 %   ReAct \cite{yao2023react} & 9.03 & 28.67  \\
     ReAct \cite{yao2023react} & 19.65 & 42.75  \\
 

 
   % ReAct \cite{yao2023react} &  &   \\

    DecomP \cite{khot2023decomposed} & 22.66 & 44.62 \\
   % DsPy \cite{khattab2023dspycompilingdeclarativelanguage} & & \\
   % SearChain \cite{xu2024searchinthechaininteractivelyenhancinglarge} & 17.07 & 30.92 \\
   %SearChain + re-rank & 19.72& 41.75 \\ 

        SearChain \cite{xu2024searchinthechaininteractivelyenhancinglarge} & 25.71& 45.16  \\ 
    

            \self{} \cite{self_ask} & 24.84 & 45.83 \\

%\self{} + re-rank & 24.44& 44.08 \\

  %  \self{} + re-rank + MER & 24.84& 45.75 \\
    

   %     \self{} + re-retrieval & 24.84& 45.75 \\
    %    \self{} + re-retrieval + MER & 26.99& 47.75 \\
        \hline
                 \colorg \textbf{NAR (w/ query understanding) (ours)}& \colorg& \colorg& \colorg\\

        $\name{}_{R}$ & 28.11 & 47.67\\  
       %   Adaptive Retrieval + MER & 31.79 & 52.5\\
        \name{} & \textbf{32.75} $\dagger$& \textbf{54.83}$\dagger$ \\
        


     
     \bottomrule
    \end{tabular}
        \caption{Results across datasets where baselines employ re-ranking for each sub-question after first-stage retrieval. The model used for \name{} and other approaches is gpt-3.5-turbo unless otherwise specified.$\dagger$ indicates statistical significance over \self{} at 0.1 level.}
    \label{tab:ranking}
\end{table}


==> tables/table_reasoning_sunar.tex <==
\begin{table}[!t]
    \small
    \centering

    \begin{tabular}{lccc}
    \toprule
     \textbf{Method}& \multicolumn{1}{c}{MQA}& \multicolumn{1}{c}{\wqa{}}\\

     % & cover-EM & cover-EM& EM& EM&EM \\
     \midrule
          \colorg \textbf{w/o \name{}} & \colorg& \colorg& \colorg\\

        ReAct &  21.41 & 43.25  \\
SearChain & 21.72 & 44.42 \\
              \colorg \textbf{w/ \name{}} & \colorg& \colorg& \colorg\\

        ReAct & 28.67 & 48.40 \\

      SearChain & \textbf{30.43} & \textbf{55.50} \\
     
     \bottomrule
    \end{tabular}
    \caption{Performance comparison when augmenting \name{} to other approaches (gpt-3.5-turbo).}
    \vspace{-2pt}
    \label{tab:reasoning_substrates}
\end{table}

